Network Topology Inference from Spectral Templates

We address the problem of identifying a graph structure from the observation of signals defined on its nodes. Fundamentally, the unknown graph encodes direct relationships between signal elements, which we aim to recover from observable indirect relationships generated by a diffusion process on the graph. The fresh look advocated here permeates benefits from convex optimization and stationarity of graph signals, in order to identify the graph shift operator (a matrix representation of the graph) given only its eigenvectors. These spectral templates can be obtained, e.g., from the sample covariance of independent graph signals diffused on the sought network. The novel idea is to find a graph shift that, while being consistent with the provided spectral information, endows the network with certain desired properties such as sparsity. To that end we develop efficient inference algorithms stemming from provably-tight convex relaxations of natural nonconvex criteria, particularizing the results for two shifts: the adjacency matrix and the normalized Laplacian. Algorithms and theoretical recovery conditions are developed not only when the templates are perfectly known, but also when the eigenvectors are noisy or when only a subset of them are given. Numerical tests showcase the effectiveness of the proposed algorithms in recovering social, brain, and amino-acid networks.

==> sec_1_introduction.tex <==
%!TEX root = Topology_inference.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: INTRODUCTION - LET'S MOTIVATE THIS THING!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{S:Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Advancing a holistic theory of networks necessitates fundamental breakthroughs in modeling,
identification, and controllability of distributed network processes -- often conceptualized as \emph{signals defined on the vertices of a graph}~\cite{barrat2012book,kolaczyk2009book}.
Under the assumption that the signal properties are related to the topology of the graph where they are supported, the goal of graph signal processing (GSP) is to develop algorithms that fruitfully leverage this relational structure~\cite{EmergingFieldGSP,SandryMouraSPG_TSP13}.
Instrumental to that end is the so-termed graph-shift operator (GSO)~\cite{SandryMouraSPG_TSP13}, a matrix capturing the graph's local topology and whose eigenbasis is central to defining graph Fourier transforms~\cite{SandryMouraSPG_TSP14Freq}. Most GSP works assume that the GSO (hence the graph) is known, and then analyze how the algebraic and spectral characteristics of the GSO impact the properties of the signals and filters defined on such a graph. Here instead we take the reverse path and investigate how to use information available from graph signals to infer the underlying graph topology; see also~\cite{DongLaplacianLearning,MeiGraphStructure,SSAMGMAR_ssp16,pasdeloup2016inferenceTSIPN16,Kalofolias2016inference_smoothAISTATS16}. 

Our focus in this paper is on identifying graphs that explain the structure of a random signal, meaning that there exists a diffusion process in the GSO that can generate the observed signal. Alternatively, we can say that the goal is to recover the GSO which encodes direct relationships between the elements of the signal from observable indirect relationships generated by a diffusion process. Such a problem is shown to be underdetermined and related to the concept of stationarity of graph signals~\cite{marques2016stationaryTSP16, perraudinstationary2016}. More precisely, it is established that the sought GSO must have the same eigenvectors as the signal's covariance matrix. This motivates a novel two-step network topology inference approach whereby we: i) leverage results from GSP theory to identify the GSO's eigenbasis from realizations of the diffused signal; and ii) rely on these (possibly imperfect and incomplete) \emph{spectral templates} to recover the GSO by estimating its eigenvalues. 

Network topology inference from a set of (graph-signal) observations is a prominent problem in Network Science~\cite{kolaczyk2009book,sporns2012book}. Since networks encode similarities between nodes, several approaches infer the so-termed \emph{association networks} by constructing graphs whose edge weights correspond to correlations or coherence measures indicating a nontrivial level of association between signal profiles at incident nodes~\cite[Ch. 7.3.1]{kolaczyk2009book}. 
%To find a sparse connectivity structure, small values are typically thresholded. 
This approach is not without merit and widely used in practice, but it exhibits several drawbacks, the main one being that links are formed taking into account only pairwise interactions, ignoring that the observed correlations can be due to latent network effects. Acknowledging these limitations, alternative methods rely on partial correlations~\cite{GLasso2008,kolaczyk2009book}, Gaussian graphical models~\cite{Lake10discoveringstructure, slawski2015estimation,meinshausen06,pavez_laplacian_inference_icassp16}, structural equation models~\cite{BazerqueGeneNetworks,BainganaInfoNetworks}, Granger causality~\cite{Brovelli04Granger,sporns2012book}, or their nonlinear (kernelized) variants~\cite{Karanikolas_icassp16,shen2016kernelsTSP16}.  Differently, recent GSP-based network inference frameworks postulate that the network exists as a latent underlying structure, and that observations are generated as a result of a network process defined in such graph. For instance, network structure is estimated in~\cite{MeiGraphStructure}  to unveil unknown relations among nodal time series adhering to an autoregressive model involving graph-filter dynamics. A factor analysis-based approach is put forth in~\cite{DongLaplacianLearning} to infer graph Laplacians, seeking that input graph signals are smooth over the learned topologies; see also~\cite{Kalofolias2016inference_smoothAISTATS16}. Different from~\cite{DongLaplacianLearning,MeiGraphStructure, Kalofolias2016inference_smoothAISTATS16} that operate on the graph domain, the goal here is to identify graphs that endow the given observations with desired spectral (frequency-domain) characteristics. Two works have recently explored this approach and addressed the problem of identifying a GSO based on its eigenvectors. One is \cite{SSAMGMAR_ssp16}, which assumes perfect knowledge of the spectral templates. The other is \cite{pasdeloup2016inferenceTSIPN16}, which only focuses on a Laplacian~GSO. 
%This paper broadens the existing results by: i) devising algorithms robust to imperfections in the templates; ii) providing theoretical results on the size of the set of feasible shifts as well as on the tightness of the sparsity-promoting, convex $\ell_1$-norm relaxations; iii) considering both adjacency and Laplacian shifts; and iv) proposing different sources for the spectral templates.

After surveying the required GSP background, in Section \ref{S:prelim_problem} we formulate the problem of identifying a GSO that explains the fundamental structure of a random signal diffused on a graph. The novel idea is to search among all feasible networks for the one that endows the resulting graph-signal transforms with prescribed spectral properties (those guaranteeing graph stationarity~\cite{marques2016stationaryTSP16}), while the inferred graph also exhibits desirable structural characteristics such as sparsity or minimum-energy edge weights. It is argued that the required spectral templates can be pragmatically obtained, e.g., via principal component analysis (PCA) of an ensemble of graph signals resulting from network diffusion dynamics. \green{Additional} sources for the spectral templates are provided in Section \ref{Ss:remark_templates}. Using the templates as input, a fairly general optimization problem is then formulated to identify the network structure. For concreteness, emphasis is laid on the recovery of two particular GSOs; namely the adjacency matrix and the normalized graph Laplacian, but our methodology can be applied to other matrix representations of graphs. In Section \ref{Ss:size_feasible_set} we derive conditions under which the feasible set of the optimization problem reduces to a singleton, a situation in which pursuit of additional network structure is rendered vacuous. When multiple solutions exist, provably-tight convex relaxations -- leading to computationally-efficient algorithms -- are developed to identify the sparsest GSO consistent with the given eigenspace  (Section \ref{Ss:relaxation}). We then introduce an inference method for the pragmatic case where knowledge of the spectral templates is imperfect (Section \ref{Ss:ShiftRecImperfEig}), and establish that the proposed algorithm can identify the underlying network topology robustly. Last but not least, in Section \ref{Ss:ShiftRecIncompEig} we investigate the case where only a subset of the GSO's eigenvectors are known. Such incomplete spectral templates arise, for example, when the observed graph signals are bandlimited. Comprehensive numerical tests corroborate our theoretical findings and confirm that the novel approach compares favorably with respect to: (i)
established methods based on (partial) correlations; and (ii) recent graph signal processing-based topology inference algorithms (Section \ref{S:Simulations}). Test cases include the recovery of social and structural brain networks, as well as the identification of the structural properties of proteins from a graph of mutual information of the co-variation of the constitutional amino-acids \cite{Marks2011proteins}.   %Concluding remarks are given in Section \ref{S:Conclusions}. 


%\newline
\noindent\emph{Notation:} The entries of a matrix $\mathbf{X}$ and a (column) vector $\mathbf{x}$ are denoted by $X_{ij}$ and $x_i$. \red{I removed the notation $[]_i$, make sure we do not use it.}
%; however, when contributing to avoid confusion, the alternative notation $[\mathbf{X}]_{ij}$ and $[\mathbf{x}]_i$ is used. 
\blue{Sets will be denoted by calligraphic capital letters and $\bbX_{\ccalI}$ will denote a submatrix of $\bbX$ formed by selecting the rows of $\bbX$ specified by $\ccalI$. }
The notation $^T$ and $^\dag$ stands for transpose and pseudo-inverse, respectively; $\mathbf{0}$ and $\mathbf{1}$ refer to the all-zero and all-one vectors. For a vector $\bbx$, $\diag(\mathbf{x})$ is a diagonal matrix \blue{whose $(i,i)$-th entry is $x_i$}; when applied to a matrix, $\diag(\bbX)$ is a vector with the diagonal elements of $\bbX$. The notation $\circ$, $\otimes$, and $\odot$ refers to the Hadamard (elementwise), Kronecker, and Khatri-Rao (columnwise Kronecker) matrix products. $\| \bbX \|_p$ denotes the $\ell_p$ norm of the \textit{vectorized} form of $\bbX$, whereas $\| \bbX \|_{M(p)}$ is the matrix norm induced by the vector $\ell_p$ norm.







==> sec_2_problem_formulation.tex <==
%!TEX root = Topology_inference.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: GRAPH SP 101, INCLUDING DIFFUSION PROCESSES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries and Problem Statement}\label{S:prelim_problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After a quick overview of the different GSP tools that will be used throughout the paper, we describe how the spectral templates can be obtained from realizations of network diffusion processes. This will allow us to formulate the network topology inference problem, the main goal of this section.
%In this section we introduce notation and terminology  as well as different GSP tools that will be leveraged through the manuscript, including the mathematical definition of a graph signal, the graph shift operator, a graph filter, and the Graph Fourier Transform (GFT).  

\subsection{Graph signal processing background}\label{Ss:gsp_background}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%x
\noindent\textbf{Graphs.} Let $\ccalG$ denote an undirected graph with a set of nodes $\mathcal{N}$ (with cardinality $N$) and a set of links $\ccalE$, such that if node $i$ is connected to $j$, then both $(i,j)$ and $(j,i)$ belong to $\ccalE$. The set $\mathcal{N}_i:=\{j\:|(j,i)\in\mathcal{E}\}$ stands for the neighborhood of $i$. 
For any given $\mathcal{G}$ we define the adjacency matrix $\bbA\in\mathbb{R}^{N\times N}$ as a sparse matrix with non-zero elements $A_{ij}=A_{ji}$ if and only if $(i,j)\in\ccalE$. The values of $A_{ji}$ can be binary, or real in the weighted case to capture the strength of the connection from $i$ to $j$. Matrix $\bbA$ can be used to define the degree vector $\bbd:=\bbA\bbone$ and the degree matrix $\bbD:=\diag(\bbd)$. Moreover, the normalized Laplacian matrix is $\bbL:=\bbI - \bbD^{-1/2} \bbA\bbD^{-1/2}\in\mathbb{R}^{N\times N}$, which is positive semidefinite and has eigenvector $\sqrt{\bbd}:=\bbD^{1/2}\mathbf{1}$ with associated eigenvalue zero. 

\noindent\textbf{Graph signals and shift operator.} 
Graph signals defined on the nodes of $\ccalG$ are functions $f : \mathcal{N} \to \mathbb{R}$, equivalently represented as vectors $\mathbf{x}=[x_1,...,x_N]^T \in  \mathbb{R}^N$, where $x_i$ denotes the signal value at node $i$. Since $\bbx$ does not account explicitly for the structure of the graph where the signal is defined, $\mathcal{G}$ is endowed with the so-called GSO $\mathbf{S}$ \cite{SandryMouraSPG_TSP13,SandryMouraSPG_TSP14Freq}. The shift $\mathbf{S}\in\mathbb{R}^{N\times N}$ is a matrix whose entry $S_{ij}$ can be non-zero only if $i=j$ or if $(i,j)\in\mathcal{E}$. The sparsity pattern of  $\bbS$ captures the local structure of $\ccalG$, but we make no specific assumptions on the values of its non-zero entries. The shift $\mathbf{S}$ can also be understood as a linear transformation that can be computed locally at the nodes of the graph. More rigorously, if $\mathbf{y}$ is defined as $\mathbf{y}=\mathbf{S}\mathbf{x}$, then node $i$ can compute $y_i$ provided that it has access to the value of $x_j$ at $j\in \mathcal{N}_i$.
%\label{Foot:footnote1}}.
Typical choices for $\mathbf{S}$ are the adjacency matrix $\bbA$ \cite{SandryMouraSPG_TSP13,SandryMouraSPG_TSP14Freq}, the (normalized) Laplacian $\bbL$~\cite{EmergingFieldGSP}, and their respective generalizations \cite{godsil2001algebraic}. %We assume henceforth that $\bbS$ is symmetric, so that $\bbS=\bbV\bbLambda\bbV^{T}$ with $\bbLambda\in\mathbb{R}^{N\times N}$ being diagonal, but our results hold for any normal GSO. 
We assume henceforth that $\bbS$ is normal, so that $\bbS=\bbV\bbLambda\bbV^{H}$ with $\bbLambda\in\mathbb{R}^{N\times N}$ being diagonal.
%In particular, $\bbS$ is diagonalizable when it is normal, i.e., it satisfies $\bbS\bbS^H=\bbS^H\bbS$. In that case we have that $\bbV$ is unitary, which implies $\bbV^{-1}=\bbV^{H}$, and leads to the decomposition $\bbS=\bbV\bbLambda\bbV^H$.

\noindent\textbf{Graph filters.} The shift $\bbS$ can be used to define linear, shift-invariant graph-signal \emph{operators} of the form
%
\begin{eqnarray}\label{E:Filter_input_output_time}
&\mathbf{H}:=\sum_{l=0}^{L-1}h_l \mathbf{S}^l&
\end{eqnarray}
%
which are called \emph{graph filters} \cite{SandryMouraSPG_TSP13}. For a given input $\bbx$, the output of the filter is simply $\bby=\bbH\bbx$. The coefficients of the filter are collected into $\mathbf{h}:=[h_0,\ldots,h_{L-1}]^T$, with $L-1$ denoting the filter degree. Graph filters are of particular interest because they represent linear transformations that can be implemented locally~\cite{segarra2015reconstruction,ssamar_distfilters_allerton15}.


\noindent\textbf{Frequency domain representation.} Leveraging the spectral decomposition of $\bbS$, graph filters and signals can be represented in the frequency domain.
To be precise, let us use the eigenvectors of $\bbS$ to define the $N\times N$ matrix $\bbU:=\bbV^T$, and the eigenvalues of $\bbS$ to define the $N\times L$ Vandermonde matrix $\bbPsi$, where $\Psi_{ij}:=(\Lambda_{ii})^{j-1}$.
Using these conventions, the frequency representations of a \emph{signal} $\bbx$ and of a \emph{filter} $\bbh$ are defined as $\widehat{\bbx}:=\bbU\bbx$ and $\widehat{\bbh}:=\bbPsi\bbh$, respectively~\cite{SandryMouraSPG_TSP14Freq}. 
Exploiting such representations, the filter's output $\bby\!=\!\bbH\bbx$ in the frequency domain is ($\odot$ denotes Hadamard product)
%
\begin{equation}\label{E:Filter_input_output_freq}
\widehat{\bby}=\diag\big(\bbPsi\bbh\big)\bbU \bbx=\diag\big(\widehat{\bbh}\big)\widehat{\bbx}=\widehat{\bbh}\odot\widehat{\bbx}.
\end{equation}
%
This identity  is the counterpart of the celebrated convolution theorem for temporal signals, and follows from $\mathbf{H}=\bbV\big(\sum_{l=0}^{L-1}h_l \boldsymbol{\Lambda}^l\big)\bbU$ [cf. \eqref{E:Filter_input_output_time}] and $\sum_{l=0}^{L-1}h_l \boldsymbol{\Lambda}^l=\diag{(\bbPsi\bbh)}$; see e.g., \cite{SSGMAMAR_camsap15} for a detailed derivation.
To establish further connections with the time domain, let us consider the directed cycle graph whose adjacency matrix $\mathbf{A}_{dc}$ is zero, except for entries $A_{ij}=1$ whenever $i=\mymod(j)+1$, where
$\mymod(x)$ denotes the modulus (remainder) obtained after dividing $x$ by $N$. If $\bbS=\bbA_{dc}$, one can verify that: i) $\bby=\bbH\bbx$ can be found as the circular convolution of $\bbh$ and $\bbx$, and ii) both $\bbU$ and $\boldsymbol{\Psi}$ correspond to the Discrete Fourier Transform (DFT) matrix. Interestingly, while in the time domain $\bbU=\boldsymbol{\Psi}$, this is not true for general graphs.

\noindent\textbf{Network diffusion processes.} Graph filters can be used to model network diffusion processes. %that depend on the network topology. To be mathematically precise, 
Specifically, the signal at node $i$ during the step $(l+1)$ of a linear diffusion process can be written as
%
\begin{eqnarray}
\label{E:local_diffusion_singlenode}
&x_i^{(l+1)}=\alpha_{ii} x_{i}^{(l)} + \sum_{j\in \ccalN_i} \alpha_{ij} x_{j}^{(l)}&
\end{eqnarray}
%
where % we recall that $\ccalN_i$ stands for the neighborhood of $i$ and 
$\alpha_{ij}$ are the diffusion coefficients; see e.g.,~\cite{SSGMAMAR_camsap15}. Leveraging the GSP framework, \eqref{E:local_diffusion_singlenode} implies that the graph signal $\bbx^{(l+1)}=\bbS\bbx^{(l)}$ at iteration $l+1$ is the shifted version of $\bbx^{(l)}$, for a shift $\bbS$ with entries  $S_{ij}=\alpha_{ij}$ if either $i=j$ or $(i,j) \in \ccalE$, and $S_{ij}=0$ otherwise.
%where the shift operator $\bbS$ is defined as: $S_{ij}:=\alpha_{ij}$, if $i=j$ or if $(i,j)\in \ccalE$; and $S_{ij}:=0$, otherwise. 
For instance, if we set $\bbS=\bbI - \beta \bbL$ and let the signal of interest be $\bbx := \bbx^{(\infty)}$, then $\bbx$ solves the heat diffusion equation~\cite{segarra2015reconstruction,SSGMAMAR_camsap15}. However, more complex diffusion dynamics such as $\bbx=\Pi_{l=0}^{\infty}(\bbI-\beta_l \bbS)\bbx^{(0)}$ and $\bbx=\sum_{l=0}^{\infty}\gamma_l \bbx^{(l)}=\sum_{l=0}^{\infty}\gamma_l \bbS^l\bbx^{(0)}$, could also be of interest. 

The Cayley--Hamilton theorem guarantees that the aforementioned infinite-horizon processes can be equivalently described by a filter of degree $N$.
Accordingly, several works have recognized that the steady-state signal $\bbx$ generated by a diffusion process can be modeled as the output of a graph filter $\bbH=\sum_{l=0}^{N-1}h_l \bbS^l$ with input (seed) $\bbx^{(0)}$~\cite{segarra2015reconstruction,SSGMAMAR_camsap15}.
The same holds true for diffusion dynamics that evolve for a finite number of steps. 
This key insight can be used to relate the statistical and spectral properties of $\bbx$ and $\bbH$ (hence the graph topology via $\bbS$). Since the eigenvectors of $\bbH$ and $\bbS$ are the same, the idea is to leverage such a relation to estimate $\bbV$. These spectral templates will then be used to identify $\bbS$ itself. 

\noindent\textbf{Obtaining the spectral templates.} Suppose that we are given a collection of $P$ steady-state signals $\{\bbx_p\}_{p=1}^P$ diffused via  \eqref{E:local_diffusion_singlenode}, and our goal is to use them to identify the eigenvectors $\bbV$. Since the signals are obtained after linearly combining successive applications of $\bbS$ to the seeding signal, one would expect the statistical properties of $\bbx$ to depend on $\bbx^{(0)}$ and the GSO $\bbS$. To be more rigorous, suppose that $\bbx^{(0)}$ is white (with identity covariance matrix) and zero mean, and let $\bbC_x:=\E{\bbx\bbx^H}$. Then, we have that 
%
\begin{align}\label{E:cov_output_filter}
\nonumber \bbC_x&=\EE\Big[\bbH\bbx^{(0)}\big({\bbx^{(0)}}\big)^H\bbH^H\Big]=\bbH \EE\Big[\bbx^{(0)}\big({\bbx^{(0)}}\big)^H\Big]\bbH^H\\
&=\bbH\bbH^H\stackrel{\star}{=}\bbV\diag(|\widehat{\bbh}|^2)\bbV^H,
\end{align}
%
where for equality $\stackrel{\star}{=}$ we leveraged the frequency interpretation of a graph filter. Identity \eqref{E:cov_output_filter} not only reveals that the color of $\bbx$ is given by the filter $\bbH$, but also that the eigenvectors of $\bbC_x$ and the shift $\bbS$ coincide. This latter assertion is true even if the filter coefficients are random, as long as they are independent of the input signal $\bbx^{(0)}$. Suppose that $\bbC_x$ is available or that it can be estimated via sample averaging to yield $\hat{\bbC}_x= 1/P\sum_{p=1}^P \bbx_p \bbx_p^H$. Then, one can use PCA (the eigendecomposition of $\hat{\bbC}_x$) to estimate the eigenvectors of $\bbS$, which will serve as input for the algorithms in the ensuing sections. %Sections \ref{S:ShiftInfFullEigen} and \ref{S:ShiftRecImperfEig} (with $K=N$). 
In closing, we mention that the aforementioned procedure is valid for any stationary graph process~\cite{marques2016stationaryTSP16}, which subsume diffusion processes driven by white noise as a special case. Additional sources for the spectral templates are outlined in Remark \ref{remark_templates}.

\subsection{Problem formulation}\label{Ss:problem_formulation}

Given $\bbV=[\bbv_1,\ldots,\bbv_N]$, we formulate the network topology inference problem as
%
	\begin{align}\label{E:general_problem} 
	\min_{ \{\bbS, \bblambda\}} \;\; f( \bbS, \bblambda) \quad \text{s. to }\;\bbS=\textstyle\sum_{k =1}^N \lambda_k\bbv_k \bbv_k^T, \,\, \bbS \in \ccalS,
	\end{align}
	%
where the optimization variables are effectively the eigenvalues $\bblambda=[\lambda_1,...,\lambda_N]^T$, since the constraint $\bbS=\sum_{k =1}^N \lambda_k\bbv_k \bbv_k^T$ forces the given templates $\bbV$ to be the eigenvectors of $\bbS$. This way, all feasible networks endow the resulting graph-signal transforms with prescribed spectral properties (cf. the definition of graph Fourier transform). The constraint set $\ccalS$ imposes certain requirements on the sought GSO, such as $\bbS$ being symmetric for undirected graphs. The objective $f$ promotes additional network structural properties which could be desirable for the application at hand, such as sparsity or minimum-energy edge weights. Note that by definition, $\bbS$ encodes the local structure of the graph it represents, thus, its recovery implies a successful identification of the graph topology of interest.

We outline four possible choices of the cost function $f$, which are intimately related to different topological and spectral features of the graph to be recovered. We first consider $f_1(\bbS) = \| \bbS \|_0$ that promotes the recovery of sparse graphs, i.e., graphs with the minimum feasible number of edges. This can be of interest in settings where $\bbS$ represents statistical dependencies among nodes, and the target is to find the most parsimonious (hence interpretable) set of relationships between those interacting elements. Related benefits of sparse graphs when it comes to large-scale network visualization are also well documented~\cite[Ch. 3]{kolaczyk2009book}. In addition, sparsity is also pertinent when $\bbS$ represents the topology of an actual network and the goal is to find a configuration that minimizes the number of active links.  Secondly, one could adopt $f_2(\bbS) = \| \bbS \|_\mathrm{F}$, which minimizes the total energy stored in the weights of the edges. As a third criterion we consider $f_3(\bbS) = \| \bbS \|_\infty$, associated with graphs of uniformly low edge weights. This can be meaningful when identifying graphs subject to capacity constraints in each link. Finally, we envision minimizing $f_4(\bblambda) = -\lambda_2$, where $\lambda_2$ is the second smallest eigenvalue and the sought GSO is assumed to be a Laplacian matrix. In this case, the recovery algorithm will promote solutions with good mixing conditions~\cite{chung1997spectral}.

The constraint $\bbS \in \ccalS$ in \eqref{E:general_problem} has a twofold motivation: a) incorporating a priori knowledge about $\bbS$; and b) preventing the trivial solution $\bbS=\bbzero$. 
%As can be seen from \eqref{E:SparseAdj_l00_obj}, when all eigenvectors $\{\bbv_k\}_{k=1}^N$ are given the design of $\bbS$ amounts to finding the $N$ eigenvalues in $\bblambda$. 
If we let $\bbS = \bbA$ represent the adjacency matrix of an undirected graph with non-negative weights and no self-loops, we can explicitly write $\ccalS$ as follows
%
\begin{align} \label{E:SparseAdj_def_S}
\ccalS_{\mathrm{A}} \!:= \! \{ \bbS \, | \, S_{ij}\!\in\! [0,1], \;  \bbS\!\in\!\ccalM^N\!\!,\;  S_{ii} = 0, \; S_{i'j'} \! = \! \alpha_{i'j'} \},
\end{align}
%
where $ij$ span all values in $\ccalN \times \ccalN$ and $i'j'$ only a subset $\ccalI$ of these.
The first condition in $\ccalS_{\mathrm{A}}$ encodes the fact that $\bbS$ is an adjacency matrix with non-negative weights, thus, every entry of $\bbS$ must lie between $0$ and an arbitrary normalization constant which we fix to $1$. The second condition incorporates the fact that the unknown graph is undirected, hence, $\bbS$ must belong to the set $\ccalM^N$ of real and symmetric $N \! \times \! N$ matrices. The third condition in $\ccalS$ encodes that the graph has no self-loops, thus, each diagonal entry of $\bbS$ must be null. Finally, the last condition in \eqref{E:SparseAdj_def_S} incorporates potential a priori knowledge on $\bbS$ by assuming that we know the nonzero values $0 \!< \! \alpha_{i'j'} \! \leq \! 1$ that $\bbS$ takes for (possibly multiple) indices $i'j'$. We assume that at least one nonzero entry of $\bbS$ is known a priori, which conveniently rules out the undesirable solution $\bbS = \mathbf{0}$ of problem \eqref{E:general_problem}. For cases where we have no a priori knowledge of specific entries of $\bbS$, the trivial solution $\bbS = \mathbf{0}$ can be avoided by, e.g., imposing $\bbS \mathbf{1} \geq \bbbeta$ which assumes that every node has a minimum degree of connectivity with its neighbors.

Alternatively, the proposed formulation can be extended to accommodate shifts $\bbS$ other than the adjacency matrix by  modifying the set $\ccalS$ in \eqref{E:general_problem} to account for the properties of the particular GSO.  Consider a scenario where $\bbS = \bbL$ represents a normalized Laplacian \cite{EmergingFieldGSP}, then the associated $\ccalS_{\mathrm{L}}$ would be
%
\begin{align}\label{E:def_S_normalized_laplacian}
\ccalS_{\rm L} \!\! := \! \{ \bbS \, | \, S_{ij}\! \in\! [-\!1, 0]   \,\, \text{for} \,\,& i\!\neq\! j,  \;\;\bbS\! \in \! \ccalM_{+}^N, \nonumber \\
&S_{ii}\!=\!1 \, \forall \, i, \,\, \lambda_1 = 0 \} .
\end{align}
%
In $\ccalS_{\rm L}$ we impose that $\bbS$ is symmetric and positive semi-definite, that its diagonal entries are $1$ and its off-diagonal entries are non-positive. Moreover, since $\bbS$ is a normalized Laplacian we know that the vector $\sqrt{\bbd}$ containing as entries the square roots of the degrees of the graph is an eigenvector whose associated eigenvalue is zero, and this is incorporated in the last constraint. Notice that for this last constraint to be implementable we should be able to identify $\sqrt{\bbd}$ among all the spectral templates in the basis $\bbV$. This can be readily done since $\sqrt{\bbd}$ is the only eigenvector whose entries have all the same sign \cite{biyikougu2007laplacian}. In the same way that a priori knowledge helps in discarding the solution $\bbS = \mathbf{0}$ for adjacency matrices, the last constraint $\lambda_1 = 0$ rules out the uninformative solution $\bbS = \bbI$ from the feasible set $\ccalS_{\rm L}$.

Naturally the identification of GSOs different from the adjacency and the normalized Laplacian can be of interest as well, including for instance the combinatorial Laplacian and the random walk Laplacian \cite{chung1997spectral}. These can be accommodated in our proposed framework via minor modifications to the set $\ccalS$. For concreteness, we henceforth focus exclusively on adjacency and normalized Laplacian matrices.

\begin{remark}[Additional sources for the spectral templates]\normalfont\label{remark_templates}
The overarching theme here is to obtain the spectral templates from PCA of a collection of signals generated by a diffusion process on a graph. Notwithstanding, impact of this paper's network topology inference approach [cf. \eqref{E:general_problem}] permeates beyond this particular use case. Accordingly, one could envision additional means of acquiring the spectral templates needed. One example in the context of distributed algorithms is the implementation of a prescribed linear network operator using a graph filter~\cite{ssamar_distfilters_allerton15}. A necessary condition to accomplish this goal is that the eigenvectors of the shift and those of the linear transformation should be the same; see \cite[Prop. 1]{ssamar_distfilters_allerton15} for details. Since the latter are given and hence serve as spectral templates, results in this paper allow one to find the sparsest GSO which facilitates implementation of a prescribed network operator via distributed graph filtering. Another example is in the context of orthonormal signal transforms. Expressing signals in an alternative domain by using a particular orthonormal transformation $\bbT$ -- such as a wavelet basis -- is known to often provide processing advantages. However, the implications of that transformation in the original domain are not always clear. In this context, solving \eqref{E:general_problem} with $\bbV^T=\bbT$ yields a shift $\bbS$ that reveals those relationships among (latent) nodes which are implicitly assumed by the transformation $\bbT$.  
\end{remark}








==> sec_2_problem_formulation_ale.tex <==
%!TEX root = Topology_inference.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: GRAPH SP 101, INCLUDING DIFFUSION PROCESSES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Statement}\label{S:prelim_problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A weighted and undirected graph $\ccalG$ consists of a node set $\ccalN$ of known cardinality $N$, an edge set $\ccalE$ of unordered pairs of elements in $\ccalN$, and edge weights $A_{ij}\in\reals$ such that $A_{ij}=A_{ji}\neq 0$ for all $(i,j)\in\ccalE$. The edge weights $A_{ij}$ are collected as entries of the adjacency matrix $\bbA$ and the node degrees in the diagonal matrix $\bbD:=\diag(\bbA\bbone)$. These are used to form the combinatorial Laplacian matrix $\bbL_c:=\bbD-\bbA$ and the normalized Laplacian $\bbL:=\bbI - \bbD^{-1/2} \bbA\bbD^{-1/2}$. More broadly, one can define a generic \blue{GSO} $\bbS\in\reals^{N\times N}$ as any matrix having the same sparsity pattern of $\ccalG$~\cite{SandryMouraSPG_TSP13}. Although the choice of $\bbS$ can be adapted to the problem at hand, most existing works set it to either $\bbA$, $\bbL_c$ or $\bbL$. 

The main focus in this paper is on identifying graphs that explain the structure of a random signal. Formally, let $\bbx=[x_1,...,x_N]^T \in\mbR^N$ be a graph signal in which the $i$th element $x_i$ denotes the signal value at node $i$ of an unknown graph $\ccalG$ with shift operator $\bbS$. Further suppose that we are given a zero-mean white signal $\bbw$ with covariance matrix $\E{\bbw\bbw^T} = \bbI$. We say that the graph $\bbS$ represents the structure of the signal $\bbx$ if there exists a diffusion process in the GSO $\bbS$ that produces the signal $\bbx$ from the white signal $\bbw$, that is
%
\begin{align}\label{eqn_diffusion}
   \bbx\  =\ \alpha_0 \prod_{l=1}^{\infty} (\bbI-\alpha_l \bbS) \bbw
       \  =\ \sum _{l=0}^{\infty} \beta_l \bbS^l \bbw .
    %   \ :=\  \bbH \bbw.
\end{align}
%
%Multiplication or summation of recursively shifted versions of the input $\bbw$ implies that the one-hop relationships encoded into $\bbS$ percolate through the entire network. 
While $\bbS$ encodes only one-hop interactions, each successive application of the shift percolates (correlates) the original information across an iteratively increasing neighborhood; see e.g.~\cite{segarra2015graphfilteringTSP15}. 
%When the number of applications of the shift exceeds the diameter of the graph, the information successfully percolates across the entire network~\cite{segarra2015graphfilteringTSP15}. 
The product and sum representations in \eqref{eqn_diffusion} are common -- and equivalent -- models for the generation of random signals. Indeed, any process that can be understood as the linear propagation of a white input through a \blue{static} graph can be written in the form in \eqref{eqn_diffusion}. 
%\blue{More generally, any process that is stationary with respect to the shift $\bbS$ can be modeled using \eqref{eqn_diffusion}; see~\cite{marques2016stationaryTSP16}.} 
These include processes generated by graph filters with time-varying coefficients or those generated by the so-called \textit{diffusion} Laplacian \textit{kernels} \cite{smola2003kernels}, to name a few. 

The justification to say that $\bbS$ is the structure of $\bbx$ is that we can think of the edges of $\bbS$ as direct (one-hop) relationships between the elements of the signal. The diffusion in \eqref{eqn_diffusion} percolates the originally white information across the network, generating indirect relationships \blue{in $\bbx$}. Our goal is to recover the fundamental relationships described by $\bbS$ from a set $\ccalX:=\{\bbx_p\}_{p=1}^P$ of $P$ independent samples of the random signal $\bbx$. We show next that this is an underdetermined problem.
%, which is closely related to the notion of stationary signals on graphs~\cite{marques2016stationaryTSP16}.
Begin by assuming that the shift operator $\bbS$ is symmetric. Define then the eigenvector matrix $\bbV=[\bbv_1,\ldots,\bbv_N]$ and the eigenvalue matrix $\bbLam=\diag(\lam_1,\ldots,\lam_N)$ to write
%
\begin{align}\label{eqn_shift_operator_normal}
\bbS =\bbV\bbLam\bbV^T.
\end{align}
%
Further observe that while the diffusion expressions in \eqref{eqn_diffusion} are polynomials on the GSO of possibly infinite degree, the Cayley-Hamilton theorem implies they are equivalent to polynomials of degree smaller than $N$. Upon defining the vector of coefficients $\bbh:=[h_0,\ldots,h_{L-1}]^T$ and the graph filter $\bbH\in\reals^{N\times N}$ as $\bbH:=\sum_{l=0}^{L-1} h_l \bbS^l$, the generative model in \eqref{eqn_diffusion} can be rewritten as
%
\begin{align}\label{E:Filter_input_output_time}
   \bbx  = \bigg(\sum_{l=0}^{L-1}h_l \bbS^l\bigg)\,\bbw
        = \bbH \bbw
\end{align}
%
for some particular $\bbh$. \red{I did not include Gonchi's comment of saying $\bbh$ and $L$ because $L$ is given by the length of $L$, but I am ok if we finally include it.} Since a graph filter $\bbH$ is a polynomial on $\bbS$~\cite{SandryMouraSPG_TSP13}, graph filters are linear graph-signal operators that have the \textit{same eigenvectors} as the shift (i.e., the operators $\bbH$ and $\bbS$ commute). More important for the present paper, the filter representation in \eqref{E:Filter_input_output_time} can be used to show that \emph{the eigenvectors of $\bbS$ are also eigenvectors of the covariance matrix $\bbC_x:=\E{\bbx\bbx^T}$.} To that end, substitute \eqref{E:Filter_input_output_time} into the covariance matrix definition and use the fact that $\E{\bbw\bbw^T} = \bbI$ to write
%
\begin{align}\label{E:cov_output_filter}
   \bbC_x = \E{\bbH\bbw\big(\bbH\bbw\big)^T}
          = \bbH \E{\bbw\bbw^T}\bbH^T
          = \bbH\bbH^T .
\end{align}
%
If we further use the spectral decomposition of the shift in \eqref{eqn_shift_operator_normal} to express the filter as $\bbH = \sum_{l=0}^{L-1} h_l (\bbV\bbLam\bbV^T)^l =\bbV(\sum_{l=0}^{L-1} h_l \bbLam^l)\bbV^T$, we can write the covariance matrix as
%
\begin{align}\label{eqn_diagonalize_covariance}
   \bbC_x\  =\ \bbV\,\bigg|\sum_{l=0}^{L-1}h_l\bbLam^l\bigg|^2\,\bbV^T
         \ :=\ \bbV\diag(\bbp)\bbV^T,
\end{align}
%
where the matrix squared-modulus operator $|\cdot|^2$ should be understood entrywise, and we have defined the vector $\bbp:=\diag(|\sum_{l=0}^{L-1}h_l\bbLam^l|^2)$ in the second equality.


The expression in  \eqref{eqn_diagonalize_covariance} is precisely the requirement for a \blue{graph} signal to be stationary \cite[Def. 3]{marques2016stationaryTSP16}; hence, the problem of identifying a GSO that explains the fundamental structure of $\bbx$ is equivalent to identifying a shift on which the signal $\bbx$ is stationary.
%
In this context, $\bbp$ is termed the power spectral density of the signal $\bbx$ with respect to $\bbS$. A consequence of this fact, which also follows directly from \eqref{eqn_diagonalize_covariance}, is that the \textit{eigenvectors} of the shift $\bbS$ and the covariance $\bbC_x$ are the same. Alternatively, one can say that the difference between $\bbC_x$, which includes indirect relationships between components, and $\bbS$, which includes exclusively direct relationships, is only on their \textit{eigenvalues}. While the diffusion in \eqref{eqn_diffusion} obscures the eigenvalues of $\bbS$, the eigenvectors $\bbV$ remain present in $\bbC_x$ as templates of the original spectrum.

Identity \eqref{eqn_diagonalize_covariance} also shows that the problem of finding a GSO that generates $\bbx$ from a white input $\bbw$ with unknown coefficients [cf. \eqref{eqn_diffusion}] is \emph{underdetermined}. As long as the matrices $\bbS$ and $\bbC_x$ have the same eigenvectors, filter coefficients that generate $\bbx$ through a diffusion process on $\bbS$ exist.\footnote{To simplify exposition, the general description of the recovery problem in this section assumes that neither $\bbS$ nor $\bbC_x$ have repeated eigenvalues. Technical modifications in the formulation to accommodate for setups where the eigenvalues are not all distinct are discussed in Section \ref{Ss:ShiftRecIncompEig}.} In fact, the covariance matrix $\bbC_x$ itself is a GSO that can generate $\bbx$ through a diffusion process and so is the precision matrix $\bbC_x^{-1}$. To sort out this ambiguity, which amounts to selecting the eigenvalues of the shift, we assume that the GSO of interest is optimal in some sense. To be more precise, let $\ccalS$ be a convex set that defines the type of shift operator we want to identify (details on $\ccalS$ are provided in Section \ref{Ss:AprioriInfoShift}) and let $\|\bbS\|_0$ count the number of nonzero entries in the GSO. We then want to identify $\bbS_0^*\in\ccalS$ with the smallest number of nonzero entries
%
\begin{alignat}{2}\label{eqn_zero_norm} 
   \bbS_0^* := &\argmin_{\{\bbS, \bblambda\}} \
                   &&\|\bbS\|_0 ,                                    \nonumber\\ 
              &\text{s. to } && \bbS = \bbV\bbLam\bbV^T 
                           = \sum_{k=1}^N \lambda_k\bbv_k \bbv_k^T,  \qquad
                      \bbS \in \ccalS,
\end{alignat}
%
where $\bblambda=[\lambda_1,\ldots,\lambda_N]^T$. To simplify notation we have purposely ignored the optimal eigenvalues $\bblambda^*_0$ that belong to the argument of the minimum. Also, we have written $\bbV\bbLam\bbV^T \! =\! \sum_{k=1}^N \lambda_k\bbv_k \bbv_k^T$ to emphasize that if the eigenvectors $\bbv_k$ are known, the constraints in \eqref{eqn_zero_norm} are linear on the unknown eigenvalues $\lam_k$. Alternatively, we can introduce criteria in the form of generic convex functions $f ( \bbS, \bblambda)$ and define the shift operator that is optimal with respect to these criteria
%
\begin{alignat}{2}\label{E:general_problem} 
   \bbS^* := &\argmin_{\{\bbS, \bblambda\}} \
                   && f ( \bbS, \bblambda),                           \nonumber\\ 
              &\text{s. to } && \bbS = \bbV\bbLam\bbV^T 
                           = \sum_{k=1}^N \lambda_k\bbv_k \bbv_k^T,  \qquad
                      \bbS \in \ccalS.
\end{alignat}
%
Possible convex choices for the criteria in \eqref{E:general_problem} are to: (i) Adopt $f(\bbS, \bblambda) = f(\bbS) = \| \bbS \|_\mathrm{F}$ which finds a GSO that minimizes the total energy stored in the weights of the edges. (ii) Make $f ( \bbS, \bblambda) = f(\bbS) = \| \bbS \|_\infty$ which yields shifts $\bbS$ associated with graphs of uniformly low edge weights. This can be meaningful, e.g., when identifying graphs subject to capacity constraints. (iii) Minimize $f ( \bbS, \bblambda) = f(\bblambda) = -\lambda_2$, where $\lambda_2$ is the second smallest eigenvalue of $\bbS$. If the GSO is further assumed to be a Laplacian matrix, this yields a shift operator that promotes solutions with fast mixing times \cite{chung1997spectral}.

Independently of the criteria, the definitions in \eqref{eqn_zero_norm} and \eqref{E:general_problem} provide a formal description of a GSO $\bbS$ that is considered to be the best possible description of the structure of the signal $\bbx$. Our goal is to find estimators of these operators as described in the following two formal problem statements.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   B   L   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{problem}\label{problem_known_matrix}
Given a covariance matrix $\bbC_x$ identify the optimal description of the structure of $\bbx$ in the form of the graph-shift operator $\bbS_0^*$ defined in \eqref{eqn_zero_norm} or $\bbS^*$ defined in \eqref{E:general_problem}.
\end{problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   B   L   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{problem}\label{problem_data_driven}
Given a set $\ccalX:=\{\bbx_p\}_{p=1}^P$ of $P$ independent samples of the random signal $\bbx$ estimate the optimal description of the structure of $\bbx$ in the form of the graph-shift operator $\bbS_0^*$ defined in \eqref{eqn_zero_norm} or $\bbS^*$ defined in \eqref{E:general_problem}.
\end{problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Problem \ref{problem_known_matrix} is a simple convex optimization problem in the case of the convex objectives in \eqref{E:general_problem} but necessitates relaxations in the case of the minimum zero-norm formulations in \eqref{eqn_zero_norm}. To solve Problem \ref{problem_known_matrix} we use (ensemble) covariance matrices to obtain the eigenvectors and show that the estimation of the eigenvalues yields consistent estimators of sparse network structures. Problem \ref{problem_known_matrix} is addressed in Section \ref{S:ShiftInfFullEigen}. To solve Problem \ref{problem_data_driven} we first use independent samples of the random signal to estimate the covariance eigenvectors via e.g., PCA. Then we estimate the eigenvalues using reformulations of \eqref{eqn_zero_norm} and \eqref{E:general_problem} which are robust to errors stemming from the aforementioned eigenvector estimation step; see Section \ref{S:ShiftInfSubsetEigen} for a detailed treatment of Problem \ref{problem_data_driven}. Although Problem \ref{problem_known_matrix} can be thought as a prerequisite to study Problem \ref{problem_data_driven}, Section \ref{Ss:remark_templates} illustrates \green{other} situations in which the estimation of a GSO with prescribed eigenvectors is of practical interest. 
%Before closing this section, a couple important remarks are in order.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{remark}[Precision matrices]\label{rmk_precision} \normalfont
As already mentioned, the precision matrix $\bbC_x^{-1} \! = \! \bbV\bbLambda^{-1}\bbV^T$ is a possible solution to the problem of finding a GSO that explains the structure of $\bbx$. This establishes a clear connection between \eqref{eqn_zero_norm} and the problem of finding sparse estimates of precision matrices~\cite[Ch. 7]{kolaczyk2009book}. If the precision matrix $\bbC_x^{-1}$ is the {\it sparsest} matrix that explains the structure of $\bbx$, this matrix is also the solution \blue{to} \eqref{eqn_zero_norm} and we have $\bbS_0^* = \bbC_x^{-1}$. In general, however, $\bbC_x^{-1}$ may not be sparse and, even if it is, there may be {\it sparser} graphs that explain  $\bbx$. In these cases the solution \blue{to} \eqref{eqn_zero_norm} is a more parsimonious GSO and we can then think of \eqref{eqn_zero_norm} as a {\it generalization} of the problem of finding a sparse precision matrix.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\begin{remark}[Spectral templates]\label{rmk_templates} \normalfont
%\red{Given a graph signal $\bbx$ and a normal shift $\bbS=\bbV\bbLambda\bbV^H$, the signal $\tilde{\bbx}:=\bbV^H\bbx$ is referred to as the
%frequency representation of $\bbx$, with $\bbV^H$ being the graph Fourier
%transform (GFT)~\cite{SandryMouraSPG_TSP14Freq}. From this vantage point, the eigenvectors $\bbV$ can 
%be interpreted as \emph{spectral templates} from which one can generate feasible shifts explaining the structure of $\bbx$ [i.e., by searching over $\bblambda$ in the network topology inference formulations \eqref{eqn_zero_norm} and \eqref{E:general_problem}]. 
%Accordingly, in addition to stationarity the graphs identified here endow the given signal observations with desired 
%frequency-domain representations.}
%\end{remark}

\subsection{A priori knowledge about the GSO}\label{Ss:AprioriInfoShift}

The constraint $\bbS \in \ccalS$ in \eqref{eqn_zero_norm}  and \eqref{E:general_problem} incorporates a priori knowledge about $\bbS$. % and prevents the trivial solution $\bbS=\bbzero$. 
%As can be seen from \eqref{E:SparseAdj_l00_obj}, when all eigenvectors $\{\bbv_k\}_{k=1}^N$ are given the design of $\bbS$ amounts to finding the $N$ eigenvalues in $\bblambda$. 
If we let $\bbS = \bbA$ represent the adjacency matrix of an undirected graph with non-negative weights and no self-loops, we can explicitly write $\ccalS$ as follows
%
\begin{align} \label{E:SparseAdj_def_S}
\ccalS_{\mathrm{A}} \!:= \! \{ \bbS \, | \, S_{ij} \geq 0, \;\,  \bbS\!\in\!\ccalM^N\!\!,\;\,  S_{ii} = 0, \;\, \textstyle\sum_j S_{j1} \! = \! 1 \}.
\end{align}
%
The first condition in $\ccalS_{\mathrm{A}}$ encodes the non-negativity of the weights whereas the second condition incorporates the fact that the unknown graph is undirected, hence, $\bbS$ must belong to the set $\ccalM^N$ of real and symmetric $N \! \times \! N$ matrices. The third condition encodes the absence of self-loops, thus, each diagonal entry of $\bbS$ must be null. Finally, the last condition fixes the scale of the admissible graphs by setting the weighted degree of the first node to $1$, and also rules out the trivial solution $\bbS\!=\!\bbzero$.  Naturally, the choice of the first node is (almost) arbitrary; any node with at least one neighbor in the sought graph suffices. Although not considered here, additional sources of information such as knowing the existence (or not) of particular edges can be incorporated into $\ccalS$ as well. 
% incorporates potential a priori knowledge on $\bbS$ by assuming that we know the nonzero values $0 \!< \! \alpha_{i'j'} \! \leq \! 1$ that $\bbS$ takes for (possibly multiple) indices $i'j'$. We assume that at least one nonzero entry of $\bbS$ is known a priori, which conveniently rules out the undesirable solution $\bbS = \mathbf{0}$ of problem \eqref{E:general_problem}. For cases where we have no a priori knowledge of specific entries of $\bbS$, the trivial solution $\bbS = \mathbf{0}$ can be avoided by, e.g., imposing $\bbS \mathbf{1} \geq \bbbeta$ which assumes that every node has a minimum degree of connectivity with its neighbors.

Alternatively, 
%the proposed formulation can be extended to accommodate shifts $\bbS$ other than the adjacency matrix by  modifying the set $\ccalS$ in \eqref{E:general_problem} to account for the properties of the particular GSO.  
when $\bbS = \bbL$ represents a normalized Laplacian \cite{EmergingFieldGSP}, the associated $\ccalS_{\mathrm{L}}$ is
%
\begin{align}\label{E:def_S_normalized_laplacian}
\ccalS_{\rm L} \!\! := \! \{ \bbS \, | \, S_{ij}\! \in\! [-\!1, 0]   \,\, \text{for} \,\,& i\!\neq\! j,  \;\;\bbS\! \in \! \ccalM_{+}^N, \nonumber \\
&S_{ii}\!=\!1 \,\, \forall \,\, i, \,\,\, \lambda_1 = 0 \} .
\end{align}
%
In $\ccalS_{\rm L}$ we impose that $\bbS$ is symmetric and positive semi-definite, its diagonal entries are $1$ and its off-diagonal entries are non-positive. Moreover, since $\bbS$ is a normalized Laplacian we know that the vector $\sqrt{\bbd}$ containing as entries the square roots of the node degrees is an eigenvector whose associated eigenvalue is zero, and this is incorporated into the last constraint. Notice that for this last constraint to be implementable we should be able to identify $\sqrt{\bbd}$ among all the spectral templates in $\bbV$. This can be done since $\sqrt{\bbd}$ is the only eigenvector whose entries have all the same sign \cite{biyikougu2007laplacian}. In the same way that fixing a scale discards the solution $\bbS = \mathbf{0}$ for adjacency matrices, the constraint $\lambda_1 = 0$ rules out the uninformative solution $\bbS = \bbI$ from the feasible set $\ccalS_{\rm L}$.

Naturally, the identification of other GSOs can be of interest as well, including for instance the combinatorial Laplacian $\bbL_c$ 
and the random walk Laplacian~\cite{chung1997spectral}. These can be accommodated in our proposed framework via minor modifications to the set $\ccalS$. For concreteness, we henceforth focus exclusively on adjacency and normalized Laplacian matrices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Additional sources for the spectral templates}\label{Ss:remark_templates} 

Since the central focus of this paper is in solving Problem \ref{problem_data_driven}, the natural source for the spectral templates is the PCA decomposition of a collection of available signals. Notwithstanding, impact of this paper's network topology inference approach [cf.~\eqref{E:general_problem}] permeates beyond that particular case. 
Three additional applications in the context of GSP, along with the corresponding sources for the templates, are provided next. 
%Accordingly, one could envision additional means of acquiring the spectral templates needed. Three relevant examples are provided next.


\subsubsection{GSO associated with orthogonal transformations}\label{ssec_AddSourcesGFT}
Expressing signals in an alternative domain by using a particular orthonormal transformation $\bbT$ -- such as wavelets or discrete-cosine bases -- has well-documented merits in \blue{a number of} signal and information processing applications. However, the implications of these transformations in the original signal domain are often unclear. To contribute to this understanding, \green{recall that a fundamental GSP assumption is that properties of the signal are related to the structure of the network. Accordingly,} the decomposition $\bbS = \bbV \bbLambda \bbV^T$ is used to define the frequency representation of the signal $\bbx$ as $\tilde{\bbx} := \bbV^T\bbx$, with $\bbV^T$ being the graph Fourier
transform (GFT)~\cite{SandryMouraSPG_TSP14Freq}. \blue{Hence, the approach proposed} here is to take the reverse path and solve \eqref{eqn_zero_norm} with $\bbV^T=\bbT$. This yields a shift $\bbS$ that helps to explain the relationships among signal elements that are implicitly assumed by the transformation $\bbT$. 


\subsubsection{Design of graph filters}\label{sssec_linearoperators}
 In addition to describing linear diffusion dynamics [cf. \eqref{E:Filter_input_output_time}], graph filters are of particular interest because they represent linear transformations that can be implemented in a distributed fashion~\cite{segarra2015reconstruction, EUSIPCO_our_interp_2015,ssamar_distfilters_allerton15}. In the context of distributed algorithms, consider implementing a prescribed linear network operator $\bbB$ using a graph filter $\bbH=\sum_{l=0}^{N-1}h_l\bbS^l$~\cite{segarra2015graphfilteringTSP15}. A necessary condition to accomplish this goal is that the eigenvectors of the shift $\bbS = \bbV \bbLambda \bbV^T$ and those of the linear transformation $\bbB = \bbV_\bbB \bbLambda_\bbB \bbV_\bbB^T$ coincide; see \cite[Prop. 1]{segarra2015graphfilteringTSP15} for details. Since $\bbV_\bbB$ can be obtained from the prescribed $\bbB$, the problems in \eqref{eqn_zero_norm} and \eqref{E:general_problem} can be solved using $\bbV=\bbV_\bbB$ as input. Hence, results in this paper enable us to find the sparsest $\bbS$ which facilitates implementation of a given network operator $\bbB$ via distributed graph filtering. 

 


\subsubsection{Graph sparsification and network deconvolution}\label{sssec_sparsify}

Given a GSO $\bbS'=\bbV\bbLambda'\bbV^T$, we can use our framework to obtain a different shift $\bbS$ with the same eigenvectors than $\bbS'$ but with desirable properties encoded in $\ccalS$ and $f(\bbS,\bblambda)$ [cf. \eqref{E:general_problem}]. \red{No implemente del todo la propuesta de Gonchi, me gusta enfatizar mas lo de graph sparsification.} \green{If we set $f(\bbS,\bblambda)=\|\bbS\|_0$, this problem falls into the class of graph sparsification, which amounts to solving \eqref{eqn_zero_norm} using as inputs the eigenvectors of $\bbS'$. Moreover, this approach can be used for the related network deconvolution task~\cite{FeiziNetworkDeconvolution},} where $\bbS'$ is the adjacency matrix of a graph encoding observed dependencies between nodes and the goal is to keep only the direct dependencies while discarding the indirect ones. Note that, different from the setup in Problem \ref{problem_known_matrix}, the matrix $\bbS'$ is not \green{necessarily} a covariance matrix. Using $\bbS$ to represent the direct dependencies among the data, the authors in~\cite{FeiziNetworkDeconvolution} model $\bbS'$ as
%
\begin{equation}\label{E:netdecov}
\bbS' = \bbS \, (\bbI + \bbS)^{-1},
\end{equation}
%
and try to identify $\bbS$ given $\bbS'$. Although they do not use this lexicon, expression \eqref{E:netdecov} models $\bbS'$ as a single-pole single-zero graph filter. We follow a more general approach where we assume that indeed $\bbS'$ can be written as a polynomial of $\bbS$, but we are agnostic to the form of the filter (polynomial coefficients). Hence, with the objective of inducing sparsity to identify the direct dependencies, we solve problem \eqref{eqn_zero_norm} where $\bbV$ is given by the eigenvectors of $\bbS'$. This general approach outperforms the network deconvolution algorithm proposed in~\cite{FeiziNetworkDeconvolution}, as demonstrated in Section \ref{Ss:Sim_network_sparsification}.

%Note that the problem of finding a canonical shift is related with that in Section \ref{ssec_AddSourcesGFT} ($\bbS'$ is used as source to identify $\bbT$), while the problem of network deconvolution is similar to that in Section \ref{sssec_linearoperators} (setting $\bbH=\bbS'$).





==> sec_3_top_inf_exact.tex <==
%!TEX root = Topology_inference.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: SHIFT INFERENCE BASED ON SPECTRAL TEMPLATES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Topology inference from spectral templates}\label{S:ShiftInfFullEigen}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As discussed in the previous section, the goal is to find a graph shift $\bbS$ that is diagonalized by the given spectral templates $\bbV=[\bbv_1,\ldots,\bbv_N]$. 
In the absence of additional constraints the problem is ill-posed, so we further impose conditions on $\bbS$ via the set $\ccalS$ % -- such as non-negative edge weights or no self-loops -- 
and search for the shift that minimizes a pre-specified cost $f$ [cf.~\eqref{E:general_problem}]. % -- such as the number of edges or the total energy of the edge weights.

The structure of the feasible set in \eqref{E:general_problem} plays a critical role towards solving our network topology inference problem. The reason is twofold. First, notice that both sets $\ccalS_{\rm A}$ and $\ccalS_{\rm L}$ are convex. Hence,  convexity of problem \eqref{E:general_problem} depends exclusively on the choice of the objective $f(\bbS,\bblambda)$, a key property to facilitate the solution of \eqref{E:general_problem} in practice. If $f(\bbS,\bblambda)$ is chosen to be convex -- e.g., equal to $\|\bbS\|_p$ with $p\geq 1$ -- the overall optimization will be convex too. Second, the dimension of the feasible set is generally small. In fact, it can be shown that in a number of setups the feasible set reduces to a singleton, or otherwise to a low-dimensional subspace. This is important because even if the objective is non-convex, searching over a small space need not be necessarily difficult.  

We first investigate the size of the feasible set and provide conditions under which it reduces to a singleton thus rendering $f$ inconsequential to the optimization. Then, for the cases where there are multiple feasible solutions, we focus on the sparsity-promoting formulation, i.e., $f(\bbS,\bblambda)=\|\bbS\|_0$.  The resultant optimization is non-convex and in fact NP-hard, so we propose computationally-efficient convex relaxations which are provably tight under some technical conditions.

\subsection{Size of the feasibility set}\label{Ss:size_feasible_set}

The feasible set of problem \eqref{E:general_problem} for both $\ccalS_{\mathrm{L}}$ and $\ccalS_{\mathrm{A}}$ is in general small. To be more precise, some notation must be introduced. Define $\bbW  \! := \! \bbV  \odot \bbV \! \in \! \reals^{N^2 \! \times \! N}$, where $\odot$ denotes the Khatri-Rao product. Notice that from the definition of $\bbS$ we can write $\bbs := \mathrm{vec}(\bbS)$ as $\bbs = \bbW \bblambda$. Hence, each row of $\bbW$ represents the $N$ weighting coefficients that map $\bblambda$ to the corresponding entry of $\bbS$. Further, define the set $\ccalD$ containing the indices of $\bbs$ corresponding to the diagonal entries of $\bbS$ and select the 
corresponding rows of $\bbW$ to form $\bbW_\ccalD\!\in\!\reals^{N\times N}$. Also, define the matrix $\bbU := \bbV^{\mathbf{1}} \circ  \bbV^{\mathbf{1}}\blue{\in\! \reals^{N\times N}}$, where $\circ$ denotes the elementwise product and $\bbV^{\mathbf{1}} := [\bbone, \bbv_2, \bbv_3, \ldots, \bbv_N ]$. Using these conventions, the following result holds.

%%%%%%%%% P R O P O S I T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproposition}\label{P:Feasibility_singleton}
Assume that \eqref{E:general_problem} is feasible, then it holds that:\\
	a) If $\ccalS = \ccalS_{\mathrm{A}}$, then $\mathrm{rank}({\bbW}_{\ccalD}) \leq N - 1$. Similarly, if $\ccalS = \ccalS_{\mathrm{L}}$, then $\mathrm{rank}(\bbU) \leq N - 1$.\\
b) If $\mathrm{rank}({\bbW}_{\ccalD}) = N - 1$ when $\ccalS = \ccalS_{\mathrm{A}}$ or $\mathrm{rank}(\bbU) = N - 1$ when $\ccalS = \ccalS_{\mathrm{L}}$, then the feasible set of \eqref{E:general_problem} is a singleton. %, which is the solution to \eqref{E:SparseAdj_l00_obj}. 
\end{myproposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
We show statements a) and b) for the case $\ccalS = \ccalS_{\mathrm{A}}$. The proofs for $\ccalS = \ccalS_{\mathrm{L}}$ are analogous and thus omitted.
The key of the proof \blue{is to note} that we may write $\bbW_\ccalD \bblambda = \diag( \bbS ) = \mathbf{0}$ for all feasible $\bblambda$. Hence, feasibility implies that ${\bbW}_{\ccalD}$ is rank-deficient as stated in a).
To show b), assume that $\mathrm{rank}({\bbW}_{\ccalD}) = N - 1$ so that $\bblambda$ in $\mathrm{null}({\bbW}_{\ccalD})$ is unique up to a scaling factor. However, \blue{since one of the conditions in $\ccalS_A$ forces} the first row of $\bbS$ to sum up to $1$ [cf.~\eqref{E:SparseAdj_def_S}], this scaling ambiguity is resolved and the unique feasible $\bblambda$ (and hence $\bbS$) is obtained.
\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Proposition~\ref{P:Feasibility_singleton} offers sufficient conditions under which \eqref{E:general_problem} reduces to a feasibility problem. More specifically, when condition b) is met, the objective in \eqref{E:general_problem} is inconsequential since there exists only one feasible $\bbS$. For more general cases, however, the GSO that minimizes the particular cost function $f$ chosen is recovered. 
%The result in Proposition~\ref{P:Feasibility_singleton} is also valid for the recovery of adjacency matrices when no a priori knowledge of any entry is available and, thus, we replace the last condition in $\ccalS_{\rm A}$ by $\bbS \mathbf{1} \geq \bbbeta$. In such a case, analogous conditions to those in a) and b) hold but depending on $Q_{\bbW_\ccalD}$, the number of null singular values of $\bbW_\ccalD$.
Among the potential cost functions, the sparsity-inducing $\ell_0$ norm $f(\bbS, \bblambda) = \| \bbS \|_0$ is non-convex, thus, challenging to solve in practice. Due to the widespread interest in identifying sparse graphs \green{(e.g., of direct relationships among signal elements)}, we devote the ensuing subsection to study this latter case separately.


\subsection{Relaxation for the sparse formulation}\label{Ss:relaxation}

Many large-scale, real-world networks are sparse~\cite{kolaczyk2009book}, so it is often meaningful  to infer a sparse GSO where most of the entries in $\bbS$ are zero [cf.~\eqref{eqn_zero_norm}]. In practice, the usual approach to handle the non-convex $\ell_0$ (pseudo) norm objective in \eqref{eqn_zero_norm} is to relax it to an iteratively re-weighted $\ell_1$ norm. Specifically, with $p$ denoting an iteration index, we aim to solve a sequence $p=1,...,P$ of weighted $\ell_1$-norm minimization problems
%
\begin{align}\label{E:SparseAdj_wl11_obj}
\bbS_{\omega}^* \! := \! \argmin_{ \{\bbS, \bblambda\}}\sum_{i,j} \!\omega_{ij}(p)|S_{ij}| \quad \text{s. to } \,\bbS=\sum_{k =1}^N \! \lambda_k\bbv_k \bbv_k^T, \,\bbS \!\in\! \ccalS,
\end{align}
%
with weights $\omega_{ij}(p):=\tau/\left(|S_{ij}(p-1)|+\delta\right)$, for appropriately chosen positive constants $\tau$ and $\delta$. Intuitively, the goal of the re-weighted scheme in \eqref{E:SparseAdj_wl11_obj} is that if $|S_{ij}(p-1)|$ is small, in the next iteration the penalization $\omega_{ij}(p)$ is large, promoting further shrinkage of $S_{ij}$ towards zero \cite{candes_l0_surrogate}.

Naturally, under condition b) in Proposition~\ref{P:Feasibility_singleton} the solutions $\bbS_0^*$ of \eqref{eqn_zero_norm} and $\bbS_{\omega}^*$ of \eqref{E:SparseAdj_wl11_obj} are guaranteed to coincide given that the feasible set is reduced to a singleton. Moreover, even when condition b) is not satisfied, there exist weights $\omega_{ij}$ that guarantee the equivalence of both solutions. 
To state this formally, define the set $\ccalJ$ containing the indices identifying the support of $\bbS^*_0$ and denote by $\ccalJ^c$ its complement. Whenever $\bbS_0^*$ is the unique solution to \eqref{eqn_zero_norm}, it is not hard to establish that by setting weights in \eqref{E:SparseAdj_wl11_obj} as $\omega_{ij}=1$ for $(i,j)\in\ccalJ^c$ and $\omega_{ij}=0$ otherwise, then $\bbS_{\omega}^*$ is unique and equal to $\bbS_0^*$. 
%To show this, notice first that since the feasibility sets of \eqref{E:SparseAdj_l00_obj} and \eqref{E:SparseAdj_wl11_obj} are equivalent, $\bbS_0^*$ is feasible in \eqref{E:SparseAdj_wl11_obj}. Moreover, by construction of the weights $\omega_{ij}$ it follows that the cost associated with $\bbS_0^*$ in \eqref{E:SparseAdj_wl11_obj} is zero, proving that it is optimal. Thus, we are left to show that no other solution to \eqref{E:SparseAdj_wl11_obj} can exist. Denoting by $\bbS_{1\rm w}^*$ a generic optimal solution, since the associated cost must be null we have that $\mathrm{supp}(\bbS_{1\rm w}^*) \subseteq \mathrm{supp}(\bbS_{0}^*)$. Combining this with the fact that $\bbS_{0}^*$ is optimal in \eqref{E:SparseAdj_l00_obj}, it must be that $\mathrm{supp}(\bbS_{0}^*) = \mathrm{supp}(\bbS_{1\rm w}^*)$. Lastly, from uniqueness of $\bbS_0^*$ we must have that $\bbS_{1\rm w}^*$ is unique, as wanted.

%%%%%%%%%% P R O P O S I T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{myproposition}\label{P:Identifiability_Adjacency_Norm1}
%Let $\bbS_0^*$ be the unique solution to \eqref{E:SparseAdj_l00_obj} and set weights $\omega_{ij}$ in \eqref{E:SparseAdj_wl11_obj} as
%%
%\begin{align}\label{E:weights_reweighted}
%\omega_{ij}=
%\begin{cases}
%1 \quad\quad \text{if} \quad i,j \in \ccalJ^c, \\
%0 \quad\quad \text{if} \quad i,j \in \ccalJ.
%\end{cases}
%\end{align}
%%
% Then, the solution $\bbS_{1\rm w}^*$ to \eqref{E:SparseAdj_wl11_obj} is unique and equal to $\bbS_0^*$.
%\end{myproposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{myproof}
%Since the feasibility sets of \eqref{E:SparseAdj_l00_obj} and \eqref{E:SparseAdj_wl11_obj} are equivalent, $\bbS_0^*$ is feasible in \eqref{E:SparseAdj_wl11_obj}. Moreover, from the weights defined in \eqref{E:weights_reweighted} it follows that the cost associated with $\bbS_0^*$ in \eqref{E:SparseAdj_wl11_obj} is zero, proving that it is optimal. Thus, we are left to show that no other solution to \eqref{E:SparseAdj_wl11_obj} can exist. Denoting by $\bbS_{1\rm w}^*$ a generic optimal solution, since the associated cost must be null we have that $\mathrm{supp}(\bbS_{1\rm w}^*) \subseteq \mathrm{supp}(\bbS_{0}^*)$. Combining this with the fact that $\bbS_{0}^*$ is optimal in \eqref{E:SparseAdj_l00_obj}, it must be that $\mathrm{supp}(\bbS_{0}^*) = \mathrm{supp}(\bbS_{1\rm w}^*)$. Lastly, from unicity of $\bbS_0^*$ we must have that $\bbS_{1\rm w}^*$ is unique, as wanted.
%\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The upshot of this simple observation is that there exist optimal weights so that the sparsest solution $\bbS^*_0$ can be recovered by solving a convex optimization problem. This result confers validity to the re-weighted formulation in \eqref{E:SparseAdj_wl11_obj}, nonetheless, we can neither choose these weights without knowing $\bbS_0^*$ a priori nor there is a guarantee that the succession of weights $\omega_{ij}(p)$ converges to these optimal weights. Hence, we now focus on the derivation of theoretical guarantees for a {particular} set of weights that can be set a priori, namely, we consider the formulation in which each entry of the GSO is equally weighted. This boils down to solving the convex optimization problem
%
\begin{align} \label{E:SparseAdj_l01_obj}
	 \bbS^*_1 \! := \! \argmin_{ \{\bbS, \bblambda\}} \,\| \bbS\|_{1} \quad \text{s. to } \bbS \! = \! \textstyle\sum_{k =1}^N \lambda_k\bbv_k \bbv_k^T, \,\,\, \bbS \in \ccalS.
\end{align}
%
Interestingly, under certain conditions we can ensure that the solution $\bbS^*_1$ to the relaxed problem \eqref{E:SparseAdj_l01_obj} coincides with $\bbS^*_0$. To be more specific, \blue{define $\bbs_0^*:= \mathrm{vec}(\bbS_0^*)$,} denote by $\ccalD^c$ the complement of $\ccalD$ and partition $\ccalD^c$ into $\ccalK$ and $\ccalK^c$, \blue{with the former indicating} the positions of the nonzero entries of \blue{$\bbs_{0\ccalD^c}^*:=(\bbs_0^*)_{\ccalD^c}$, where we recall that matrix \textit{calligraphic subscripts} select rows. Denoting} by $^\dag$ the matrix pseudo-inverse, we define
%
\begin{equation}\label{E:def_matrix_M}
\bbM := (\bbI - \bbW \bbW^\dag)_{\ccalD^c}\blue{\,\in\reals^{N^2-N\times N^2}},
\end{equation}
%
i.e., the orthogonal projector onto the kernel of $\bbW^T$ \green{constrained} to the off-diagonal elements in $\ccalD^c$. With $\bbe_1$ denoting the first canonical basis vector, we construct the matrix 
%
\begin{equation}\label{E:def_matrix_R}
\bbR := [ \bbM, \, \bbe_1 \otimes \bbone_{N-1}]\blue{\,\in\reals^{N^2-N\times N^2+1}},
\end{equation}
%
by horizontally concatenating $\bbM$ and a column vector of size $|\ccalD^c|$ with ones in the first $N-1$ positions and zeros elsewhere. With this notation in place, the following recovery result holds.

%%%%%%%%%%% T H E O R E M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mytheorem}\label{T:Recovery}
Whenever $\ccalS = \ccalS_{\rm A}$ and assuming problem \eqref{E:SparseAdj_l01_obj} is feasible, $\bbS^*_1 = \bbS^*_0$ if the two following conditions are satisfied:\\
A-1) $\rank(\bbR_{\ccalK}) = |\ccalK|$; and \\   
A-2) There exists a constant $\delta > 0$ such that 
%
\begin{equation}\label{E:condition_recovery_noiseless}
{\psi_{\bbR}} := \| \bbI_{\ccalK^c}(\delta^{-2}\bbR \bbR^T+\bbI_{\ccalK^c}^T \bbI_{\ccalK^c})^{-1}\bbI_{\ccalK}^T \|_{M(\infty)}<1.
\end{equation}
\end{mytheorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
Recalling that $\bbs = \mathrm{vec}(\bbS)$, problem \eqref{E:SparseAdj_l01_obj} for the case where $\ccalS = \ccalS_{\rm A}$ can be reformulated as
%
\begin{equation}\label{E:proof_noiseless_recovery_010}
\min_{ \{\bbs, \bblambda\}} \;\; \|\bbs\|_1 \;\;\text{s. to } \;\;\bbs= \bbW \bblambda,\;\;\bbs_{\ccalD}=\bbzero,\;\;(\bbe_1 \otimes \bbone_N)^T \bbs = 1,
\end{equation}
%
where the last equality imposes that the first column of $\bbS$ must sum up to $1$ [cf.~\eqref{E:SparseAdj_def_S}]. Notice that the non-negativity constraint in $\ccalS_{\rm A}$ is ignored in \eqref{E:proof_noiseless_recovery_010}. However, if we show that \eqref{E:proof_noiseless_recovery_010} can recover the sparse solution $\bbs_0^*$, then the same solution would be recovered by the more constrained problem \eqref{E:SparseAdj_l01_obj}. Notice that we may solve for $\bblambda$ in closed form as $\bblambda^* = \bbW^{\dag} \bbs$. Consequently,  \eqref{E:proof_noiseless_recovery_010} becomes 
%
\begin{equation}\label{E:proof_noiseless_recovery_020}
\min_{\bbs} \|\bbs\|_1 \;\;\: \text{s. to } (\bbI - \bbW \bbW^\dag) \bbs = \bbzero,\;\bbs_{\ccalD}=\bbzero,\;(\bbe_1 \otimes \bbone_N)^T \bbs = 1.
\end{equation}
%
Leveraging the fact that $\bbI - \bbW \bbW^\dag$ is symmetric, the first equality in \eqref{E:proof_noiseless_recovery_020} can be rewritten as [cf.~\eqref{E:def_matrix_M}]
%
\begin{equation}\label{E:proof_noiseless_recovery_030}
(\bbI - \bbW \bbW^\dag)^T_\ccalD \bbs_{\ccalD} + \bbM^T \bbs_{\ccalD^c} = \bbzero,
\end{equation}
% 
and the second equality in \eqref{E:proof_noiseless_recovery_020} forces the first term of \eqref{E:proof_noiseless_recovery_030} to be zero. With these considerations, we may restate \eqref{E:proof_noiseless_recovery_020} as 
%
\begin{equation}\label{E:proof_noiseless_recovery_040}
\min_{ \bbs_{\ccalD^c}} \;\; \|\bbs_{\ccalD^c}\|_1 \;\;\text{s. to } \;\; \bbR^T \bbs_{\ccalD^c} = \bbb,
\end{equation}
%
where $\bbb$ \blue{is a vector of length $N^2+1$ with all its entries equal to $0$ except for the last one that is a $1$}.
Problem \eqref{E:proof_noiseless_recovery_040} takes the form of classical basis pursuit~\cite{ChenDonohoBP}. Notice that the system of linear equations in \eqref{E:proof_noiseless_recovery_040} is overdetermined since $\bbR^T \in \reals^{N^2+1 \times | \ccalD^c|}$, however, feasibility of \eqref{E:proof_noiseless_recovery_010} guarantees that the mentioned system of equations is compatible. The following two conditions are required for the solution of \eqref{E:proof_noiseless_recovery_040} to coincide with the sparse solution ${\bbs_0^*}_{\ccalD^c}$ (cf.~\cite{zhang2013one}): 
\begin{itemize}
	\item[a)] $\mathrm{ker}(\bbI_{\ccalK^c}) \cap \mathrm{ker}(\bbR^T) = \{ \mathbf{0} \}$; and
	 \item[b)] There exists a vector $\bby \in \reals^{|\ccalD^c|}$ such that $\bby \in \mathrm{Im}(\bbR)$, $\bby_\ccalK = \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK)$, and $\| \bby_{\ccalK^c}\|_\infty < 1$.
\end{itemize}

%Condition a) is required for the solution to \eqref{E:proof_noiseless_recovery_040} to be unique whereas condition b), by ensuring the existence of an appropriate dual certificate, guarantees the optimality of the solution.
\noindent The remainder of the proof is devoted to showing that if conditions \emph{A-1)} and \emph{A-2)} in the statement of the theorem hold true, then a) and b) are satisfied.

To see that \emph{A-1)} implies a) notice that the nullspace of $\bbI_{\ccalK^c}$ is spanned by the columns of $\bbI^T_{\ccalK}$. Hence, for a) to hold we need the $|\ccalK|$ columns of $\bbR^T$ in positions $\ccalK$ to form a full column rank matrix. In condition \emph{A-1)} we require $\bbR_\ccalK$ to be full row rank, which is an equivalent property.

The next step is to show that condition \emph{A-2)} implies b). For this, consider the following \blue{$\ell_2$-norm} minimization problem
%
\begin{align}\label{E:l_2_minimization_dual_certificate}
\min_{ \{\bby, \bbz\}} \; \delta^2\|\bbz\|_2^2 + \|\bby\|_2^2  \;\;\text{s. to } \; \bby= \bbR\bbz,\;\; \bby_\ccalK = \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK), 
\end{align}
%
\red{Before (in (13) and in the line before) we used the notation $()_\ccalK$, here we are using $[]_\ccalK$. We should be consistent and update the notation remark in the introduction accordingly.} where $\delta$ is a positive tuning constant. The inclusion of the term $\delta^2\|\bbz\|_2^2$ in the objective guarantees the existence of a closed-form expression for the optimal solution, while preventing numerical instability when solving the optimization. We will show that the solution $\bby^*$ to problem \eqref{E:l_2_minimization_dual_certificate} satisfies the requirements imposed in condition b). The two constraints in \eqref{E:l_2_minimization_dual_certificate} enforce the fulfillment of the first two requirements in b), hence, we are left to show that $\| \bby^*_{\ccalK^c}\|_\infty < 1$.
Since the values of $\bby_{\ccalK}$ are fixed, the constraint $\bby= \bbR \bbz$ can be rewritten as $\bbI_{\ccalK}^T \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK) = -\bbI_{\ccalK^c}^T \bby_{\ccalK^c} +  \bbR \delta^{-1} \delta\bbz$. Then, by defining the vector $\bbt := [\delta\bbz^T, -\bby_{\ccalK^c}^T]^T$ and the matrix $\bbPhi:= [\delta^{-1} \bbR^T, \bbI_{\ccalK^c}]$, \eqref{E:l_2_minimization_dual_certificate} can be rewritten as
%
\begin{align}\label{E:l_2_minimization_dual_certificate_rewritten}
\min_{\bbt} \;\; \|\bbt\|_2^2  \;\;\text{s. to } \; \bbI_{\ccalK}^T \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK) = \bbPhi^T \bbt.
\end{align}
%
The minimum-norm solution to \eqref{E:l_2_minimization_dual_certificate_rewritten} is given by $\bbt^*=(\bbPhi^T)^\dag \bbI_{\ccalK}^T \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK)$ from where it follows that
%
\begin{align}\label{E:dual_certificate_solution_norm2_delta}
\bby^*_{\ccalK^c}  \!=\!  - \bbI_{\ccalK^c}(\delta^{-2}\bbR \bbR^T+\bbI_{\ccalK^c}^T \bbI_{\ccalK^c})^{-1}\bbI_{\ccalK}^T \, \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK).
\end{align}
%
Condition a) guarantees the existence of the inverse in \eqref{E:dual_certificate_solution_norm2_delta}. Since $\| \mathrm{sign}([{\bbs_0^*}_{\ccalD^c}]_\ccalK) \|_{\infty} \! = \! 1$, we may bound the $\ell_\infty$ norm of $\bby^*_{\ccalK^c}$ as $\| \bby^*_{\ccalK^c} \|_{\infty} \leq \| \bbI_{\ccalK^c}(\delta^{-2}\bbR \bbR^T+\bbI_{\ccalK^c}^T \bbI_{\ccalK^c})^{-1}\bbI_{\ccalK}^T \|_{M(\infty)} = \psi_{\bbR}$.
Hence, condition \emph{A-2)} in the theorem guarantees $\| \bby^*_{\ccalK^c} \|_{\infty}<1$ as wanted, concluding the proof.
\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Theorem \ref{T:Recovery} offers \textit{sufficient} conditions under which the relaxation \eqref{E:SparseAdj_l01_obj} is tight, thus guaranteeing sparse recovery for adjacency and normalized Laplacian matrices. Simulations in Section~\ref{S:Simulations} reveal that the bounds imposed on $\psi_{\bbR}$ and $\psi_{\bbQ}$ are tight by providing examples where $\psi_{\bbR}$ is exactly one and for which recovery fails. In Theorem~\ref{T:Recovery}, conditions a-1) and b-1) ensure that the solution to \eqref{E:SparseAdj_l01_obj} is unique, a necessary requirement to guarantee sparse recovery. Conditions a-2) and b-2) are derived from the construction of a dual certificate specially designed to ensure that the unique solution to \eqref{E:SparseAdj_l01_obj} also has minimum $\ell_0$ norm.

Theorem~\ref{T:Recovery} offers \textit{sufficient} conditions under which the relaxation \eqref{E:SparseAdj_l01_obj} guarantees sparse recovery for adjacency matrices. Simulations in Section~\ref{S:Simulations} reveal that the bound imposed on $\psi_{\bbR}$ is tight by providing examples where $\psi_{\bbR}$ is equal to 1 and for which recovery fails. In Theorem~\ref{T:Recovery}, condition \emph{A-1)} ensures that the solution to \eqref{E:SparseAdj_l01_obj} is unique, a necessary requirement to guarantee sparse recovery. Condition \emph{A-2)} is derived from the construction of a dual certificate \red{[add ref here or at the end of the sentence]} specially designed to ensure that the unique solution to \eqref{E:SparseAdj_l01_obj} also has minimum $\ell_0$ norm.}

Recall that the $\ell_\infty$ norm in \eqref{E:condition_recovery_noiseless} is computing the maximum $\ell_1$ norm across the rows of the argument matrix, which has $|\ccalK_c|$ rows each containing $|\ccalK|$ elements. It is expected that sparser graphs (small $|\ccalK|$) might have smaller values of $\psi_{\bbR}$. In any case, to have an intuitive understanding of $\psi_{\bbR}$ it is helpful to see that condition \emph{A-2)} is always satisfied whenever the feasible set of \eqref{E:SparseAdj_l01_obj} is a singleton (cf. Proposition~\ref{P:Feasibility_singleton}). To see this, since $\bbM$ in \eqref{E:def_matrix_M} is a projector onto the kernel of $\bbW^T$\blue{, which is orthogonal to the image space of $\bbW$,} we have that $\bbM \bbs = \bbzero$ only if $\bbs$ is the vectorized form of a shift achievable by the eigenbasis $\bbV$. \red{I do not understand this, nor the following discussion, can we just say that the reason is that $\bbR\bbR^T$ is not singular. As it is, it is like explaining equations with words without a clear simplifying message.} Thus, whenever $\mathrm{rank}({\bbW}_{\ccalD}) = N - 1$, we have that $\mathrm{rank}(\bbM) = |\ccalD^c| - 1$ since the admissible shifts are restrained to a one-dimensional subspace. Furthermore, when fixing the scale by imposing the sum of the elements in the first column to be one, the feasible set becomes a singleton or, equivalently, $\bbR$ in \eqref{E:def_matrix_R} is guaranteed to be full row rank. This implies that $\bbR \bbR^T$ in \eqref{E:condition_recovery_noiseless} is non-singular so that we can make $\delta$ arbitrarily small to ensure fulfillment of condition \emph{A-2)}. \green{Characterizing the ensembles of random graphs that tend to satisfy \eqref{E:condition_recovery_noiseless} with high probability is of interest, but left as future research.}
%
%Probabilistic guarantees for the fulfillment of \eqref{E:condition_recovery_noiseless} and the characterization of classes of graphs that tend to satisfy \eqref{E:condition_recovery_noiseless} with high probability are of interest but left as future research~avenues.

The recovery result of Theorem~\ref{T:Recovery} can be replicated for the case where the shift of interest is a normalized Laplacian, i.e., when $\ccalS = \ccalS_{\rm L}$. To state this formally, if we define $\bbQ := (\bbI - \tilde{\bbU} \tilde{\bbU}^\dag)_{\ccalD^c}$, where $\tilde{\bbU} := \tilde{\bbV} \odot  \tilde{\bbV}$ for $ \tilde{\bbV} := [\bbv_2, \bbv_3, \ldots, \bbv_N]$ the following result holds. The proof follows the same steps as those in Theorem~\ref{T:Recovery} and, thus, is omitted.

%%%%%%%%%%% T H E O R E M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mytheorem}\label{T:Recovery_Laplacian}
Whenever $\ccalS = \ccalS_{\rm L}$ and assuming problem \eqref{E:SparseAdj_l01_obj} is feasible, $\bbS^*_1 = \bbS^*_0$ if the two following conditions are satisfied:\\
L-1) $\rank(\bbQ_\ccalK) = | \ccalK |$; and \\
L-2) There exists a constant $\delta > 0$ such that
%
\begin{equation}\label{E:condition_recovery_noiseless_laplacian}
{\psi_{\bbQ}} := \| \bbI_{\ccalK^c}(\delta^{-2}\bbQ \bbQ^T+\bbI_{\ccalK^c}^T \bbI_{\ccalK^c})^{-1}\bbI_{\ccalK}^T \|_{M(\infty)}<1.
\end{equation}
%
\end{mytheorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sec_4_top_inf_imperfect.tex <==
%!TEX root = Topology_inference.tex
	
	
	
	
	
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: SHIFT INFERENCE USING A SUBSET OF THE EIGENBASIS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Imperfect spectral templates}\label{S:ShiftInfSubsetEigen}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Whenever the number of observed graph signals is limited or the observations are noisy, assuming perfect knowledge of the spectral templates $\bbV$ may be unrealistic. This section broadens the scope of the network inference problems dealt with so far, to accommodate for imperfect spectral templates that can either be noisy or incomplete. Specifically, we investigate pragmatic scenarios where: i) only an approximate version of $\bbV$ can be obtained (e.g., from the eigenvectors of a \emph{sample} covariance matrix); and ii) where only a subset of $\bbV$ is available (e.g., when the observed signals are bandlimited and one can only estimate \blue{the non-zero frequencies that are present}).

\subsection{Noisy spectral templates} \label{Ss:ShiftRecImperfEig}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We first address the case where knowledge of an approximate version of the spectral templates $\hat{\bbV} = [\hat{\bbv}_1,\ldots,\hat{\bbv}_N]$ is available.
The question here is how to update the general formulation in \eqref{E:general_problem} to account for the discrepancies between the estimated spectral templates $\hat{\bbV}$ and the actual eigenvectors of $\bbS$. An instructive reformulation is to include $\bbV= [\bbv_1, \ldots, \bbv_N]$ as decision variables and formulate the following problem
%
\begin{align}\label{E:SparseAdj_l1_obj_noisy_vectors}
	&\min_{\{\bbS, \bblambda, \bbV\}} \;f( \bbS,\bblambda) \quad \\
	&\text{s. to } \,\, \bbS = \textstyle\sum_{k =1}^N \lambda_k\bbv_k \bbv_k^T, \,\,\, \bbS \in \ccalS, \,\,\, d(\bbv_k, \hat{\bbv}_k) \leq \epsilon_k \,\,\forall \, k, \nonumber
\end{align}
%
where $d(\cdot, \cdot)$ is a \textit{convex} vector distance function, such as the $\ell_p$ norm of the vector difference for $p \! \geq \! 1$. The idea in \eqref{E:SparseAdj_l1_obj_noisy_vectors} is to find a sparse $\bbS$ that satisfies the desired properties in $\ccalS$, while its eigenvectors $\bbv_k$ are each of them close to the observed ones $\hat{\bbv}_k$. The value of $\epsilon_k$ must be chosen based on a priori information on the imperfections, such as the number of signals used to estimate the sample covariance, or the statistics of the observation noise. While conceptually simple, problem \eqref{E:SparseAdj_l1_obj_noisy_vectors} is more challenging than its noiseless counterpart, since the first constraint is non-convex given that both $\lambda_k$ and $\bbv_k$ are optimization variables. 

A more tractable alternative is to form $\bbS':=\sum_{k =1}^{N} \lambda_k \hat{\bbv}_k \hat{\bbv}_k^T$ and search for a shift $\bbS$ that possesses the desired properties while being close to $\bbS'$. Formally, one can solve
%
\begin{align}\label{E:SparseAdj_l1_obj_noisy_matrix}
	\hat{\bbS}^*&:=\argmin_{\{\bbS, \bblambda, \bbS'\}} \; f( \bbS,\bblambda) \,\,\,\, \\
		&\text{s. to } \,\, \bbS' = \textstyle\sum_{k =1}^N \lambda_k \hat{\bbv}_k \hat{\bbv}_k^T, \,\,\,\, \bbS \in \ccalS, \,\,\,d(\bbS, \bbS') \leq \epsilon, \nonumber
\end{align}
%
where $d(\cdot, \cdot)$ is a \textit{convex} matrix distance whose form depends on the particular application. E.g., if $\|\bbS-\bbS'\|_\mathrm{F}$ is chosen, the focus is more on the similarities across the entries of the shifts, while $\|\bbS-\bbS'\|_{M(2)}$ focuses on their spectrum. Additional conic constraints of the form $\|(\bbS-\bbS')\hbv_k\|_2\leq \lambda_k\epsilon_k$\blue{, enforcing that particular eigenvectors are well approximated,} can also be incorporated. From an application point of view, the formulation in \eqref{E:SparseAdj_l1_obj_noisy_matrix} is also relevant to setups where the templates $\hbV$ are not necessarily noisy but the goal is to enlarge the set of feasible GSOs. This can be of interest if, for example, finding an $\bbS$ that is both sparse and with the exact templates collected in $\hbV$ is impossible \blue{(cf. Section \ref{Ss:remark_templates})}.

The difficulty in solving \eqref{E:SparseAdj_l1_obj_noisy_matrix} is determined by $f(\cdot,\cdot)$ and $\ccalS$. Hence, the challenges and approaches are similar to those in Section \ref{S:ShiftInfFullEigen}. For the particular case of sparse shifts, the $\ell_1$ norm relaxation of \eqref{E:SparseAdj_l1_obj_noisy_matrix} yields [cf. \eqref{E:SparseAdj_l01_obj}]
%
\begin{align}\label{E:SparseAdj_l1_obj_noisy_matrix_v2}
\hat{\bbS}^*_1&:=\argmin_{\{\bbS, \bblambda, \bbS'\}} \; \|\bbS\|_1 \,\,\,\, \\
&\text{s. to } \,\, \bbS' = \textstyle\sum_{k =1}^N \lambda_k \hat{\bbv}_k \hat{\bbv}_k^T, \,\,\,\, \bbS \in \ccalS, \,\,\,d(\bbS, \bbS') \leq \epsilon, \nonumber
\end{align}
%  
where iteratively re-weighted schemes are also possible. Moreover, further uncertainties can be introduced in the definition of the feasible set $\ccalS$, e.g. in the scale of the admissible graphs for the case of $\ccalS = \ccalS_{\rm A}$. As a matter of fact, this latter source of uncertainty is considered in Proposition~\ref{P:noisy_recovery} [cf.~\eqref{E:proof_noisy_recovery_005}].
 
When the interest is in recovering a normalized Laplacian [cf.~\eqref{E:def_S_normalized_laplacian}], a possible implementation is to enforce the constraint $\lambda_1 = 0$ \emph{talis qualis} on \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} entailing that one of the eigenvalues of $\bbS'$ (and not $\bbS$) is equal to zero. However, the smallest eigenvalue of $\bbS$ must be close to zero due to the constraint on the distance between $\bbS$ and $\bbS'$. Alternatively, the objective can be augmented by also considering the nuclear norm $\| \bbS \|_*$ to further promote rank-deficiency on $\bbS$.

To assess the effect of the noise in recovering the sparsest $\bbS$, we define matrices $\hbW$, $\hat{\bbR}$ and $\hat{\bbQ}$ which are \blue{counterparts} of $\bbW$, $\bbR$ and $\bbQ$ defined prior to Theorem~\ref{T:Recovery}, but based on the noisy templates $\hat{\bbV}$ instead of $\bbV$. With this notation, the following result on robust recovery of network topologies holds.
%
%%%%%%%%% P R O P O S I T I O N %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproposition}\label{P:noisy_recovery}
When $d(\bbS, {\bbS}') = \| \bbS - {\bbS}' \|_\mathrm{F}$, and assuming that there exists at least one ${\bbS}'$ such that $d(\bbS_0^*, {\bbS}')\leq \epsilon$, the solution $\hbs_1^* := \mathrm{vec}(\hbS_1^*)$ to \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} satisfies
	%
	\begin{equation}\label{E:recov_noise}
		\| \hbs_1^* - \bbs_0^* \|_1 \leq C \epsilon, \quad \text{with} \,\,\, C = 2 C_1 + 2 C_2 C_3,
	\end{equation}
	%
	if the same conditions stated in Theorems~\ref{T:Recovery} and \ref{T:Recovery_Laplacian} hold but for $\hat{\bbR}$ and $\hat{\bbQ}$ instead of ${\bbR}$ and ${\bbQ}$, respectively.
	For the case $\ccalS = \ccalS_\mathrm{A}$ with scale uncertainty, constants $C_1$, $C_2$, and $C_3$ are given by 
	%
	\begin{equation}\label{E:recov_noise_constants}
		C_1 \!=\! \frac{\sqrt{| \ccalK |}}{\sigma_{\min}(\hat{\bbR}^T_\ccalK)}, \,\, C_2 \!=\! \frac{1 + \| \hat{\bbR}^T \|_{M(2)} C_1}{1 - \psi_{\hat{\bbR}}}, \,\, C_3 \!=\! \| \hat{\bbR}^{\dag} \|_{M(2)} N,
	\end{equation}
	%
	where $\sigma_{\min}( \cdot)$ denotes the minimum singular value of the argument matrix.
	Analogous constants can be defined for the case $\ccalS = \ccalS_\mathrm{L}$ but based on $\hat{\bbQ}$ instead of $\hat{\bbR}$.
\end{myproposition}
%%%%%%%%%%%%%%%%%
\begin{myproof}
\blue{If $\ccalS = \ccalS_{\mathrm{A}}$ and we incorporate the uncertainty in the scale of admissible graphs, the problem}
%
\begin{align}\label{E:proof_noisy_recovery_005}
\min_{ \{\bbs, \bblambda, \bbs'\}} \;\; \|\bbs\|_1 \;\;\text{s. to }& \;\;\bbs'= \hbW \bblambda,\;\;\bbs_{\ccalD}=\bbzero, \\
&\|\bbs - \bbs'\|_2^2 + ((\bbe_1 \otimes \bbone_N)^T \bbs - 1)^2 \leq \epsilon^2. \nonumber
\end{align}
%
\blue{yields a solution to  \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2}.} As done in the proof of Theorem~\ref{T:Recovery}, we purposely ignore the non-negativity constraint on $\bbs$. Substituting the first equality constraint in \eqref{E:proof_noisy_recovery_005} into the inequality constraint, then solving for $\bblambda$ as $\bblambda^* = \hbW^\dag \bbs$, and finally using the second equality constraint to reduce the optimization variables to $\bbs_{\ccalD^c}$, we may restate \eqref{E:proof_noisy_recovery_005} as [cf.~\eqref{E:proof_noiseless_recovery_040}]
%
\begin{equation}\label{E:proof_noisy_recovery_010}
\min_{ \bbs_{\ccalD^c}} \;\; \|\bbs_{\ccalD^c}\|_1 \quad\; \text{s. to } \; \| \hat{\bbR}^T \bbs_{\ccalD^c} - \bbb \|_2 \leq \epsilon,
\end{equation}
%
where $\bbb$ is, as in the proof of Theorem~\ref{T:Recovery}, a vector with all its entries equal to 0 except for the last one that is equal to 1. Notice that \eqref{E:proof_noisy_recovery_010} takes the form of a basis pursuit problem with noisy observations~\cite{ChenDonohoBP}. Expressions \eqref{E:recov_noise} and \eqref{E:recov_noise_constants} can be derived by applying the second claim in \cite[Theorem~2]{zhang2013one} to problem \eqref{E:proof_noisy_recovery_010}. In order to do so, a few factors must be taken into consideration. First, since $\hat{\bbR}^T$ is not full row rank (since it is a tall matrix), constant $C_3$ depends on the $\ell_2$ norm of $\hat{\bbR}^{\dag}$. Moreover, in order to make constants $C_1$, $C_2$, and $C_3$ independent of the dual certificate $\bby \in \reals^{|\ccalD^c|}$ -- see condition b) within the proof of Theorem~\ref{T:Recovery} -- we have used that $\| \bby \|_2 \leq N $ and $\| \bby_{\ccalK^c} \|_\infty \leq \psi_{\hat{\bbR}}$, where the first one follows from the fact that the magnitude of every element in $\bby$ is at most $1$ and the second one was shown after \eqref{E:dual_certificate_solution_norm2_delta}.

A similar procedure can be used to show the result pertaining the case where $\ccalS \!= \! \ccalS_{\rm L}$.
\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When given noisy versions $\hat{\bbV}$ of the spectral templates of our target GSO, Proposition~\ref{P:noisy_recovery} quantifies the effect that the noise has on the recovery. More precisely, the recovered shift is guaranteed to be at a maximum distance from the desired shift bounded by the tolerance $\epsilon$ times a constant, which depends on $\hbR$ and the support $\ccalK$. In particular, this implies that as the number of observed signals increases we recover the true graph shift as stated in the following remark.

\begin{remark}[Consistent estimator]\label{R:consistent_estimator}\normalfont
As the number of observed signals increases the sample covariance $\hbC_x$ tends to the covariance $\bbC_x$ and, for the cases where the latter has no repeated eigenvalues, the noisy eigenvectors $\hbV$ tend to the eigenvectors $\bbV$ of the desired shift; see, e.g., \cite[Theo. 3.3.7]{Ortega90}. In particular, with better estimates $\hat{\bbV}$ the tolerance $\epsilon$ in \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} needed to guarantee feasibility can be made smaller, entailing a smaller discrepancy between the recovered $\bbS_1^*$ and the sparsest shift $\bbS_0^*$. In the limit when $\hat{\bbV} = \bbV$ and under no additional uncertainties, the tolerance $\epsilon$ can be made zero and \eqref{E:recov_noise} guarantees perfect recovery under conditions \emph{A-1)} and \emph{A-2)} in Theorem~\ref{T:Recovery} or \emph{L-1)} and \emph{L-2)} in Theorem~\ref{T:Recovery_Laplacian}.
\end{remark}




\subsection{Incomplete spectral templates} \label{Ss:ShiftRecIncompEig}

Thus far we have assumed that the entire set of eigenvectors $\bbV= [\bbv_1, \ldots, \bbv_N]$ is known, either perfectly or corrupted by noise. However, it is conceivable that in a number of scenarios only some of the eigenvectors (say $K$ out of $N$) are available. This would be the case when e.g., $\bbV$ is found as the eigenbasis of $\bbC_x$ and the given signal ensemble is bandlimited. More generally, whenever $\bbC_x$ contains repeated eigenvalues there is a rotation ambiguity in the definition of the associated eigenvectors. Hence, in this case, we keep the eigenvectors that can be unambiguously characterized and, for the eigenvectors with repeated eigenvalues, we include the rotation ambiguity as an additional constraint in our optimization problem.

Formally, assume that the $K$ first eigenvectors $\bbV_K=[\bbv_1,...,\bbv_K]$ are those which are known. Then, the network topology inference problem with incomplete spectral templates can be formulated as [cf.~\eqref{E:SparseAdj_l01_obj}] 
%
\begin{align}\label{E:SparseAdj_l00_onlysomeeig}
		\bar{\bbS}^*_1& := \argmin_{ \{\bbS, \bbS_{\bar{K}}, \bblambda\}} \;\; \| \bbS \|_1 \\
		 & \text{s. to } \;\; \bbS= \bbS_{\bar{K}} + {\textstyle\sum_{k=1}^{K}} \lambda_k \bbv_k \bbv_k^T, \;\; \bbS\in\ccalS, \;\; \bbS_{\bar{K}}\bbV_K=\bb0, \nonumber
\end{align}
%
where we already particularized the objective to the $\ell_1$ convex relaxation.
The formulation in \eqref{E:SparseAdj_l00_onlysomeeig} enforces $\bbS$ to be partially diagonalized by the known spectral templates $\bbV_K$, while its remaining component $\bbS_{\bar{K}}$ is forced to belong to the orthogonal complement of $\text{range}(\bbV_K)$. Notice that, as a consequence, the rank of $\bbS_{\bar{K}}$ is at most $N-K$. As in the previous cases, $\ccalS$ incorporates a priori information about the GSO. Notice that the constraint in $\ccalS$ imposing symmetry on $\bbS$ combined with the first constraint in \eqref{E:SparseAdj_l00_onlysomeeig} automatically enforce symmetry on $\bbS_{\bar{K}}$, as wanted.
An advantage of using only partial information of the eigenbasis as opposed to the whole $\bbV$ is that the set of feasible solutions in \eqref{E:SparseAdj_l00_onlysomeeig} is larger than that in \eqref{E:SparseAdj_l01_obj}. This is particularly important when the  templates do not come from a preexisting shift but, rather, one has the freedom to choose $\bbS$ provided it satisfies certain spectral properties. A practical example is the selection of the topology of a sensor network aimed at implementing estimation tasks -- such as consensus -- which can be oftentimes written as rank-one transformations of the sensor observations~\cite{segarra2015graphfilteringTSP15}.

Theoretical guarantees of recovery analogous to those presented in Section~\ref{Ss:relaxation} can be derived for \eqref{E:SparseAdj_l00_onlysomeeig}. To formally state these, the following notation must be introduced. Define $\bbW_K := \bbV_K \odot \bbV_K$ and $\bbUpsilon := [\bbI_{N^2}, \bbzero_{N^2 \times N^2}]$. Also, define matrices $\bbB^{(i,j)} \in \reals^{N \times N}$ for $i < j$ such that $B^{(i,j)}_{ij} = 1$, $B^{(i,j)}_{ji} = -1$, and all other entries are zero. Based on this, we denote by $\bbB \in \reals^{{N \choose 2} \times N^2}$ a matrix whose rows are the vectorized forms of $\bbB^{(i,j)}$ for all $i,j \in \{1, 2, \ldots, N\}$ where $i < j$. In this way, $\bbB \bbs = \bbzero$ when $\bbs$ is the vectorized form of a symmetric matrix. Further, we define the following matrices %with $N^2$ columns and $N^2+N+(N^2-N)/2+NK+1$ rows
%
\begin{equation}\label{E:def_P_matrices}
\bbP_1 \!:=\! 
\begin{bmatrix}
\bbI - \bbW_K \bbW_K^\dag \\
\bbI_\ccalD \\
\bbB \\
\bbzero_{NK \times N^2} \\
(\bbe_1 \otimes \bbone_N)^T 
\end{bmatrix}^T, \quad
\bbP_2 \!:=\! 
\begin{bmatrix}
\bbW_K \bbW_K^\dag - \bbI \\
\bbzero_{N \times N^2} \\
\bbzero_{{N \choose 2} \times N^2} \\
\bbI \otimes V_K^T \\
\bbzero_{1 \times N^2}
\end{bmatrix}^T,
\end{equation}
%
and $\bbP := [\bbP_1^T , \bbP_2^T]^T$. With this notation in place, and denoting by $\ccalJ$ the support of $\bbs_0^* = \mathrm{vec}(\bbS^*_0)$, the following result holds.

%%%%%%%%%%% T H E O R E M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mytheorem}\label{T:Recovery_incomplete}
Whenever $\ccalS = \ccalS_{\rm A}$ and assuming problem \eqref{E:SparseAdj_l00_onlysomeeig} is feasible, $\bar{\bbS}^*_1 = \bbS^*_0$ if the two following conditions are satisfied:\\
A-1) $\rank([{\bbP_1}_\ccalJ^T, \bbP_2^T]) = |\ccalJ| + N^2$; and \\   
A-2) There exists a constant $\delta > 0$ such that 
%
\begin{equation}\label{E:condition_recovery_incomplete}
\eta_{\bbP} := \| \bbUpsilon_{\ccalJ^c}(\delta^{-2} \bbP \bbP^T + \bbUpsilon_{\ccalJ^c}^T \bbUpsilon_{\ccalJ^c})^{-1}\bbUpsilon_{\ccalJ}^T \|_{M(\infty)}<1.
\end{equation}
\end{mytheorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{myproof}
With $\bbs = \mathrm{vec}(\bbS)$ and $\bbs_{\bar{K}} = \mathrm{vec}(\bbS_{\bar{K}})$, we reformulate \eqref{E:SparseAdj_l00_onlysomeeig} for $\ccalS = \ccalS_{\rm A}$ as
%
\begin{align}\label{E:proof_incomplete_recovery_010}
		\min_{ \{\bbs, \bbs_{\bar{K}}, \bblambda\}} & \;\; \| \bbs \|_1 \\
		  \text{s. to } \;\; &\bbs= \bbs_{\bar{K}} + \bbW_K \bblambda, \; \bbs_{\ccalD} = \bbzero, \; \bbB \bbs = \bbzero,  \nonumber \\
		 & (\bbe_1 \otimes \bbone_N)^T \bbs= 1,  \; (\bbI \otimes V_K^T)\bbs_{\bar{K}} = \bbzero. \nonumber
\end{align}
%
The first and last constraints in \eqref{E:proof_incomplete_recovery_010} correspond to the first and last constraints in \eqref{E:SparseAdj_l00_onlysomeeig} written in vector form. The second constraint in \eqref{E:proof_incomplete_recovery_010} imposes that $\bbS$ has no self-loops, the third one imposes symmetry on $\bbS$, and the fourth one normalizes the first column of $\bbS$ to sum up to 1 [cf.~\eqref{E:SparseAdj_def_S}]. Notice that the non-negativity constraint in $\ccalS_{\rm A}$ is ignored in \eqref{E:proof_incomplete_recovery_010}, however, if we show that \eqref{E:proof_incomplete_recovery_010} can recover the sparse solution $\bbs_0^*$, then the same solution would be recovered by the more constrained problem \eqref{E:SparseAdj_l00_onlysomeeig}. Using the first constraint to solve for $\bblambda$, we obtain $\bblambda = \bbW_K^\dag (\bbs - \bbs_{\bar{K}})$. Moreover, defining the concatenated variable $\bbt:= [ \bbs^T, \bbs_{\bar{K}}^T]^T$, it follows from the definitions of $\bbUpsilon$ and $\bbP$ that \eqref{E:proof_incomplete_recovery_010} can be reformulated as
%
\begin{align}\label{E:proof_incomplete_recovery_020}
		\min_{ \bbt }  \;\; \| \bbUpsilon \bbt \|_1 \quad \; \text{s. to } \;  \bbP^T \bbt = \bbb,
\end{align}
%
where $\bbb$ is a vector with every entry equal to $0$ except for the last one which is equal to $1$. We utilize existing results on $\ell_1$-analysis \cite{zhang2013one} to state that the solution to \eqref{E:proof_incomplete_recovery_020} coincides with the sparsest solution if:
\begin{itemize}
	\item[a)] $\mathrm{ker}(\bbUpsilon_{\ccalJ^c}) \cap \mathrm{ker}(\bbP^T) = \{ \mathbf{0} \}$; and
	 \item[b)] There exists a vector $\bby \in \reals^{N^2}$ such that $\bbUpsilon^T \bby \in \mathrm{Im}(\bbP)$, $\bby_\ccalJ = \mathrm{sign}({\bbs_0^*}_{\ccalJ})$, and $\|\bby_{\ccalJ^c}\|_\infty < 1$.
\end{itemize}


%%%%%%%%%%%%%%%   F   I   G   U   R    E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
	\input{figures/num_experiments.tex}	
	\vspace{-0.15in}
	\caption{(a) Proportion of topology inference problems with a unique feasible point for Erd\H{o}s-R\'enyi graphs as a function of $N$ and $p$ for adjacency (top) and normalized Laplacian (bottom) matrices. (b) Recovery rate for the same set of graphs in (a) when implementing the iteratively re-weighted approach in \eqref{E:SparseAdj_wl11_obj}. (c) Histogram of the rank of matrix $\bbU$ for $N\!=\!10$ and $p\!=\!0.2$. (d) Experimental validation of Theorem~\ref{T:Recovery}. Whenever $\psi_{\bbR} < 1$ perfect recovery is achieved.}
			\vspace{-0.1in}
	\label{F:num_exp} 
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent As was the case for Theorem~\ref{T:Recovery}, the proof now reduces to showing that conditions \emph{A-1)} and \emph{A-2)} in the statement of the theorem imply the above conditions a) and b).

From the specific form of $\bbUpsilon$, the kernel of $\bbUpsilon_{\ccalJ^c}$ is a space of dimension $|\ccalJ| + N^2$ spanned by the set of canonical basis vectors $\bbe_i$ of length $2 N^2$ where $i \in \ccalJ \cup \{N^2+1, N^2+2, \ldots, 2 N^2\}$. Thus for a) to hold we need the matrix formed by the columns of $\bbP^T$ indexed by $\ccalJ \cup \{N^2+1, \ldots, 2 N^2\}$ to be full column rank, as stated in condition \emph{A-1)}.

Finally, the procedure to show that \emph{A-2)} implies b) follows the same steps as those detailed in the proof of Theorem~\ref{T:Recovery} -- from \eqref{E:l_2_minimization_dual_certificate} onwards -- and, thus, omitted here. 
\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Theorem~\ref{T:Recovery_incomplete} offers {sufficient} conditions for the relaxed problem in \eqref{E:SparseAdj_l00_onlysomeeig} to recover the sparsest graph, even when incomplete information about the eigenvectors is available. In practice it is observed that for smaller number $K$ of known spectral templates the value of $\eta_{\bbP}$ in \eqref{E:condition_recovery_incomplete} tends to be larger, indicating a less favorable setting for recovery. This observation is aligned with the results obtained in practice; see Fig.~\ref{F:num_exp_2}(c).

To state results similar to those in Theorem~\ref{T:Recovery_incomplete} but for the recovery of normalized Laplacians, we define $\tilde{\bbU}_K := \tilde{\bbV}_K \odot  \tilde{\bbV}_K$ where $ \tilde{\bbV}_K := [\bbv_2, \bbv_3, \ldots, \bbv_K]$ and define the matrices
%
\begin{equation}\label{E:def_T_matrices}
\bbT_1 := 
\begin{bmatrix}
\bbI - \tilde{\bbU}_K \tilde{\bbU}_K^\dag \\
\bbI_\ccalD \\
\bbB \\
\bbzero_{NK \times N^2} \\
\end{bmatrix}^T, \quad
\bbT_2 := 
\begin{bmatrix}
\tilde{\bbU}_K \tilde{\bbU}_K^\dag - \bbI \\
\bbzero_{N \times N^2} \\
\bbzero_{{N \choose 2} \times N^2} \\
\bbI \otimes V_K^T \\
\end{bmatrix}^T,
\end{equation}
%
and $\bbT := [\bbT_1^T , \bbT_2^T]^T$. Under the assumption that the leading eigenvector of the normalized Laplacian, i.e. the eigenvector whose entries all have the same sign, is among the $K$ eigenvectors known the following result holds. The proof -- here omitted -- follows the same steps as those in Theorem~\ref{T:Recovery_incomplete}.


%%%%%%%%%%% T H E O R E M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mytheorem}\label{T:Recovery_incomplete_Laplacian}
Whenever $\ccalS = \ccalS_{\rm L}$ and assuming problem \eqref{E:SparseAdj_l00_onlysomeeig} is feasible, $\bar{\bbS}^*_1 = \bbS^*_0$ if the two following conditions are satisfied:\\
L-1) $\rank([{\bbT_1}_\ccalJ^T, \bbT_2^T]) = |\ccalJ| + N^2$ ; and \\
L-2) There exists a constant $\delta > 0$ such that 
%
\begin{equation}\label{E:condition_recovery_incomplete_laplacian}
\eta_{\bbT} := \| \bbUpsilon_{\ccalJ^c}(\delta^{-2} \bbT \bbT^T + \bbUpsilon_{\ccalJ^c}^T \bbUpsilon_{\ccalJ^c})^{-1}\bbUpsilon_{\ccalJ}^T \|_{M(\infty)}<1.
\end{equation}
%
\end{mytheorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%These issues will be analyzed numerically in Section \ref{S:NumResults}. 


Notice that scenarios that combine the settings in Sections~\ref{Ss:ShiftRecImperfEig} and~\ref{Ss:ShiftRecIncompEig}, i.e. where the knowledge of the $K$ templates is imperfect, can be handled by combining the formulations in \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} and \eqref{E:SparseAdj_l00_onlysomeeig}. This can be achieved upon implementing the following modifications to \eqref{E:SparseAdj_l00_onlysomeeig}: considering the shift $\bbS'$ as a new optimization variable, replacing the first constraint in \eqref{E:SparseAdj_l00_onlysomeeig} with $\bbS'=\bbS_{\bar{K}}+{\textstyle \sum_{k=1}^{K}} \lambda_k \bbv_k \bbv_k^T$, and adding $d(\bbS,\bbS') \leq \epsilon$ as a new constraint [cf.~\eqref{E:SparseAdj_l1_obj_noisy_matrix_v2}].  


	

 














==> sec_5_numerical_experiments.tex <==
%!TEX root = Topology_inference.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical experiments}\label{S:Simulations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\red{We still need to define the name of the algorithm, if any.}\green{1. NETIST - NEtwork Topology Inference based on Spectral Templates. 2. NETISP - NEtwork Topology Inference based on Spectral temPlates. 3. GRATIS - GRAph Topology Inference based on Spectral templates. 4 GRATISP - GRAph Topology Inference based on Spectral temPlates. I vote for 2, but it seems that there is a company with that name. 3 and 4 would not have that problem.}

We test the proposed topology inference methods on different synthetic and real-world graphs. A comprehensive performance evaluation is carried out whereby we: (i)~investigate the recovery of both adjacency and normalized Laplacian matrices; (ii)~corroborate our main theoretical findings; (iii)~assess the impact of imperfect information in the recovery;  (iv)~carry out comparisons with state-of-the-art methods; and (v)~illustrate how our framework can be used to promote sparsity on a given network.

\subsection{Topology inference from noiseless templates}\label{Ss:Sim_Top_inf_noiseless_templates}


Consider Erd\H{o}s-R\'enyi graphs \cite{bollobas1998random} of varying size $N \in \{10, 20, \dots, 50\}$ and different edge-formation probabilities $p \in \{0.1, 0.2, \ldots, 0.9\}$. For each combination of $N$ and $p$ we generate 100 graphs and try to recover their adjacency $\bbA$ and normalized Laplacian $\bbL$ matrices from the corresponding spectral templates $\bbV$. In Fig.~\ref{F:num_exp}(a) we plot the proportion of instances where the corresponding optimization problems -- problem \eqref{E:general_problem} for $\ccalS = \ccalS_\mathrm{A}$ and $\ccalS = \ccalS_\mathrm{L}$ -- have singleton feasibility sets. Notice that multiple solutions are more frequent when the expected number of neighbors of a given node is close to either $1$ or $N$. For intermediate values of $p$, the rank of both ${\bbW}_{\ccalD}$ and $\bbU$ is typically $N-1$, guaranteeing a single feasible point (cf. Proposition~\ref{P:Feasibility_singleton}). Using the same set of graphs that those in Fig.~\ref{F:num_exp}(a), Fig.~\ref{F:num_exp}(b) shows the recovery rate when solving the iteratively re-weighted problem \eqref{E:SparseAdj_wl11_obj} for both the adjacency (top) and the normalized Laplacian (bottom). As expected, the rates in Fig.~\ref{F:num_exp}(b) dominate those in Fig.~\ref{F:num_exp}(a) since every instance with a unique feasible point is recovered successfully. Moreover, the improved rates observed in Fig.~\ref{F:num_exp}(b) are indicative of the beneficial effect that the weighted $\ell_1$ norm objective has in the recovery.


%%%%%%%%%%%%%%%   F   I   G   U   R    E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
	\begin{minipage}[c]{.33\textwidth}
		\includegraphics[width=\textwidth]{figures/brain_for_journal.pdf}
		\centering{\small (a)}
	\end{minipage}%
	\begin{minipage}[c]{.33\textwidth}
		\includegraphics[width=\textwidth]{figures/social_noisy_for_journal.pdf}
		\centering{\small (b)}
	\end{minipage}%
	\begin{minipage}{.33\textwidth}
		\includegraphics[width=\textwidth]{figures/social_incomplete_for_journal.pdf}
		\centering{\small (c)}
	\end{minipage}
	\caption{ (a) Brain graph recovery error for three patients as a function of the number of signals observed in the estimation of the spectral templates.  (b)~Recovery error for four social networks as a function of the number of signals observed in the estimation of the spectral templates. (c) Recovery error for four social networks (with $N=32$ nodes) as a function of $K$, the number of spectral templates that are known.}
				\vspace{-0.15in}
	\label{F:num_exp_2}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As indicated by Proposition~\ref{P:Feasibility_singleton}, the rate of recovery is intimately related to the ranks of ${\bbW}_{\ccalD}$ and $\bbU$ for the adjacency and normalized Laplacian cases, respectively. Fig.~\ref{F:num_exp}(c) further illustrates this relation via a histogram of the rank of $\bbU$ for the 100 graphs with $N=10$ and $p=0.2$. For more than half of the instances, the rank of $\bbU$ is equal to 9 (blue bar) and, as stated in Proposition~\ref{P:Feasibility_singleton}, for all these graphs there is a unique feasible point (yellow bar) that is successfully recovered (cyan bar). We see that, as the rank of $\bbU$ degrades, uniqueness is no longer guaranteed but for most cases the true graph can still be recovered following the iteratively re-weighted scheme proposed. Only in 8 of the cases where $\mathrm{rank}(\bbU)<9$ the recovery was not successful, entailing a recovery rate of 0.92, as reported in the corresponding entry ($N=10$, $p=0.2$) of the bottom plot in Fig.~\ref{F:num_exp}(b).

Finally, in order to corroborate the conditions for noiseless recovery stated in Theorem~\ref{T:Recovery}, we draw Erd\H{o}s-R\'enyi random graphs of size $N \!=\! 20$ and edge-formation probability $p \! = \! 0.25$. For each graph, we make sure that the associated $\bbW_{\ccalD}$ matrix has rank strictly smaller than $N-1$ (to rule out the cases where the feasible set is a singleton), and that condition \emph{A-1)} in Theorem~\ref{T:Recovery} is satisfied. In Fig.~\ref{F:num_exp}(d) we plot the number of successes and failures in recovering the adjacency as a function of $\psi_\bbR$ in \eqref{E:condition_recovery_noiseless}. We consider 1000 realizations and for each of them the constant $\delta$ in \eqref{E:condition_recovery_noiseless} is chosen to minimize $\psi_\bbR$. Fig.~\ref{F:num_exp}(d) clearly depicts the result of Theorem~\ref{T:Recovery} in that, for all cases where $\psi_\bbR<1$, relaxation \eqref{E:SparseAdj_l01_obj} achieves perfect recovery. Equally important, it is clear that the bound stated in \eqref{E:condition_recovery_noiseless} is tight since a large proportion of the realizations with $\psi_\bbR$ equal to 1 or just above this value lead to failed recoveries.


\subsection{Topology inference from noisy and incomplete templates}\label{Ss:Sim_Top_inf_noisy_templates}

We consider the identification of unweighted and undirected graphs corresponding to human brains~\cite{hagmann2008mapping}, consisting of $N=66$ nodes or regions of interest (ROIs) and whose edges link ROIs with density of anatomical connections greater than a threshold. The threshold is chosen as the largest one that entails a connected graph. We test the recovery from noisy spectral templates $\hat{\bbV}$ [cf.~\eqref{E:SparseAdj_l1_obj_noisy_matrix_v2}] obtained from sample covariances of synthetic signals generated through diffusion processes (cf.~Section~\ref{S:prelim_problem}). 
These processes are modeled by graph filters of random degree between $3$ and $7$, and with independent and normally distributed coefficients.
Denoting by $\hat{\bbV}_i$ the noisy spectral templates of patient $i \! \in \! \{1, 2, 3\}$ and by $\hat{\bbA}_i$ the adjacency matrices recovered, Fig.~\ref{F:num_exp_2}(a) plots the recovery error as a function of the number of signals observed in the computation of the sample covariance. The error is quantified as the proportion of edges misidentified, i.e., $\|\bbA_i \!-\! \hat{\bbA}_i\|_0 / \| \bbA_i \|_0$, and each point in Fig.~\ref{F:num_exp_2}(a) is the average across 50 realizations. 
%First notice that in the noiseless case ($\sigma = 0$), perfect recovery is achieved for the three patients. 
Notice that for an increasing number of observed signals we see a monotonous decrease in recovery error. For example, when going from $10^4$ to $10^5$ observations the error is (approximately) divided by seven, when averaged across patients. This is reasonable since a larger number of observations gives rise to a more reliable estimate of the covariance matrix entailing less noisy spectral templates. 
%\blue{Notice that, even though the performance increases for all patients with the number of observations, the brain of patient 1 is consistently the hardest to identify. For instance, consider the errors for $10^5$ observations, where for patient 1 we successfully recover $96.4\%$ of the \textit{edges}, whereas for patients 2 and 3 the average recovery rate is $99.5\%$ and $99.4\%$, respectively. This points towards the fact that some graphs are inherently more robust for identification when given noisy spectral templates. A formal analysis of this phenomenon is left as future work.}
Traditional methods like graphical lasso \cite{GLasso2008} fail to recover $\bbS$ from the sample covariance of filtered white signals. 
%This occurs because, in general, the filter $\bbH$ introduces conditional dependence between signal values more than one hop apart. 
E.g., when focusing on filters of the form $\bbH = h_0 \bbI + h_1 \bbS$, graphical lasso underperforms compared to the method presented. More precisely, based on $10^5$ observations, the recovery error of graphical lasso averaged over 50 realizations and with optimal tuning parameters is 0.303, 0.350, and 0.270 for patients 1, 2, and 3, respectively [cf. Fig.~\ref{F:num_exp_2}(a)]. Further comparisons of our method with graphical lasso and other existing alternatives are detailed in Section~\ref{Ss:Sim_performance_comparison}. 

%%%%%%%%%%%%%%%   F   I   G   U   R    E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.44\textwidth]{figures/comparison_traditional_methods_v_2.pdf}
	\vspace{-0.1in}	
	\caption{Performance comparison between spectral templates (SpecTemp), graphical lasso, and correlation-based recovery. For general filters, SpecTemp outperforms the other two.}
			\vspace{-0.15in}
	\label{F:comparison_traditional}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We repeat the previous experiment on four social networks defined on a common set of nodes representing 32 students from the University of Ljubljana. Each network represents different types and levels of interactions among the students, and were built by asking each student to select a group of preferred college mates for different situations, e.g., to discuss a personal issue or to invite to a birthday party\footnote{Access to the data and additional details are available at \url{http://vladowiki.fmf.uni-lj.si/doku.php?id=pajek:data:pajek:students}}. The considered graphs are unweighted and symmetric, and the edge between $i$ and $j$ exists if either student $i$ picked $j$ in the questionnaire or vice versa. As done for the brain graphs, we test the recovery performance for noisy spectral templates $\hat{\bbV}$ obtained from sample covariances. Fig.~\ref{F:num_exp_2}(b) plots the reconstruction error as a function of the number of observed signals for the different networks studied. As was observed in Fig.~\ref{F:num_exp_2}(a), we see a monotonous decrease in recovery error for all the analyzed networks.

%\blue{Traditional methods like graphical lasso \cite{GLasso2008} fail to recover $\bbS$ from the sample covariance of filtered white signals. This happens because the filter $\bbH$ introduces conditional dependence between signal values\textit{ more than one hop} apart. For instance, based on $10^5$ observations, the recovery error of graphical lasso with optimal tuning parameters and averaged over 50 realizations is $0.548$, $0.348$, $0.313$, and $0.429$ for the four networks studied.}


%%%%%%%%%%%%%%%  T  A  B  L  E  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}
\centering
 \caption{Performance comparison between spectral templates (SpecTemp), Kalofolias \cite{Kalofolias2016inference_smoothAISTATS16}, and Dong etal \cite{DongLaplacianLearning}.}
 		\vspace{-0.1in}
 \begin{tabular}{r c c c c c c c c c c c c} 
 & & \multicolumn{3}{c}{Inverse Laplacian} & & \multicolumn{3}{c}{Diffusion} & & \multicolumn{3}{c}{Exponential} \\[1pt]
 \cline{3-5}  \cline{7-9}  \cline{11-13} \\[-6pt]
 & & SpecTemp & Kalofolias & Dong etal & & SpecTemp & Kalofolias & Dong etal & & SpecTemp & Kalofolias & Dong etal \\[1pt]
 \hline
 {\bf Erd\H{o}s-R\'enyi} & & & & & & & & & & & & \\
 F-measure &  & {\bf 0.896}  &  0.791  &  0.818 &  & {\bf 0.924}  &  0.868  &  0.828 &  & {\bf 0.703}  &  0.651  &  0.667 \\
 edge error &  & {\bf 0.108}  &  0.152  &  0.168 &  & {\bf 0.071}  &  0.149  &  0.177 &  & {\bf 0.276}  &  0.318  &  0.332 \\
 degree error & & {\bf 0.058}  &  0.071  &  0.105 & & {\bf 0.040}  &  0.055  &  0.111 & & {\bf 0.162}   & 0.201  &  0.222 \\
 {\bf Barab\'asi-Albert} & & & & & & & & & & & & \\
 F-measure & & {\bf 0.926}  &  0.855  &  0.873 & & {\bf 0.945}  &  0.845  &  0.894 & & {\bf 0.814}  &  0.732  &  0.798 \\
 edge error & & {\bf 0.143}  &  0.173  &  0.209 & & {\bf 0.135}  &  0.154  &  0.235 & & {\bf 0.310}  &  0.314  &  0.393 \\
 degree error & & {\bf 0.108}  &  0.124  &  0.169 & & 0.109  &  {\bf 0.092}  &  0.188 & & {\bf 0.240}  &  0.244  &  0.282 \\
 \hline
 \end{tabular}
  		\vspace{-0.1in}
 \label{Tab:comparison_methods}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finally, we illustrate the recovery performance in the presence of incomplete spectral templates by solving \eqref{E:SparseAdj_l00_onlysomeeig} for the aforementioned four networks. In Fig.~\ref{F:num_exp_2}(c) we plot the recovery error as a function of the number $K$ of eigenvectors available. Each point in the plot is the average across 50 realizations in which different $K$ eigenvectors were selected from the $N\!=\!32$ possible ones. As expected, performance for all networks increases with the number of spectral templates known. The performance improvement is sharp and precipitous going from a large error of over $0.85$ for three of the networks when 17 spectral templates are known to a perfect recovery for all the networks when 24 eigenvectors are given. Moreover, notice that network $4$ is consistently the easiest to identify both for noisy [cf. Fig.~\ref{F:num_exp_2}(b)] and incomplete [cf. Fig.~\ref{F:num_exp_2}(c)] spectral templates. For example, when given 19 spectral templates the error associated with network $4$ is $0.224$ whereas the average across the other three networks is $0.584$. This hints towards the fact that some graphs are inherently more robust for identification when given imperfect spectral templates. A formal analysis of this phenomenon is left as future work.


\subsection{Performance comparison}\label{Ss:Sim_performance_comparison}

We compare the performance of the presented method based on spectral templates (we refer to it as SpecTemp for conciseness) with established statistical approaches as well as recent GSP-based algorithms.

\noindent\textbf{Comparison with established methods.} We analyze the performance of SpecTemp in comparison with two widely used methods, namely, (thresholded) correlation~\cite[Ch. 7.3.1]{kolaczyk2009book}  and graphical lasso \cite{GLasso2008}. 
Our goal is to recover the adjacency matrix of an undirected and unweighted graph with no self-loops from the observation of filtered graph signals. 
For the implementation of SpecTemp, we use the eigendecomposition of the sample covariance of the observed signals in order to extract noisy spectral templates $\hat{\bbV}$. We then solve problem \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} for $\ccalS = \ccalS_{\mathrm{A}}$, where $\epsilon$ is selected as the smallest value that admits a feasible solution. We include as a priori knowledge that each node has at least one neighbor. For the correlation-based method, we keep the absolute value of the sample correlation of the observed signals, force zeros on the diagonal and set all values below a certain threshold to zero. This threshold is determined during a training phase, as explained in the next paragraph. Lastly, for graphical lasso we follow the implementation in \cite{GLasso2008} based on the sample covariance and select the tuning parameter $\rho$ (see \cite{GLasso2008}) during the training phase. We then force zeros on the diagonal and keep the absolute values of each entry. Leveraging that the sought graphs are unweighted, for SpecTemp and graphical lasso a fixed threshold of 0.3 is used so that, after recovery, every edge with weight smaller than the threshold is set to zero.


%%%%%%%%%%%%%%%   F   I   G   U   R    E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.41\textwidth]{figures/compare_Kalo_Dong_observations.pdf}
	\vspace{-0.1in}	
	\caption{Comparison of edge recovery error as a function of the number of signals observed for SpecTemp, Kalofolias \cite{Kalofolias2016inference_smoothAISTATS16}, and Dong etal\cite{DongLaplacianLearning}.}
			\vspace{-0.15in}
	\label{F:comparison_kalo_dong}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We test the recovery of adjacency matrices $\bbS \! = \! \bbA$ of Erd\H{o}s-R\'enyi (ER) graphs \cite{bollobas1998random} with $N \! = \! 20$ nodes and edge probability $p \! = \! 0.2$. We vary the number of observed signals from $10^1$ to $10^6$ in powers of $10$. Each of these signals is generated by passing white Gaussian noise through a graph filter $\bbH$. Two different types of filters are considered. 
As a first type we consider a \emph{general} filter $\bbH_1 = \bbV \diag(\widehat{\bbh}_1) \bbV^T$, where the entries of $\widehat{\bbh}_1$ are independent and chosen randomly between $0.5$ and $1.5$. 
The second type is a \emph{specific} filter of the form $\bbH_2 = (\delta \bbI + \bbS)^{-1/2}$, where the constant $\delta$ is chosen so that $\delta \bbI + \bbS$ is positive definite to ensure that $\bbH_2$ is real and well-defined. Following the discussion in Section~\ref{S:prelim_problem}, this implies that the precision matrix of the filtered signals is given by $\bbC_x^{-1} = \bbH_2^{-2} = \delta \bbI + \bbS$, which coincides with the desired GSO $\bbS$ in the off-diagonal elements. 
For each combination of filter type and number of observed signals, we generate 10 ER graphs that are used for training and 20 ER graphs that are used for testing. Based on the 10 training graphs, the optimal threshold for the correlation method and parameter $\rho$ for graphical lasso are determined and then used for the recovery of the 20 testing graphs. Given that for SpecTemp we are fixing $\epsilon$ beforehand, no training is required.


%%%%%%%%%%%%%%%   F   I   G   U   R    E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
	\centering
	\input{figures/network_sparsification.tex}	
	\vspace{-0.25in}
	\caption{(a) Real and inferred contact networks between amino-acid residues for protein BPT1 BOVIN. Ground truth contact network (top left), mutual information of the co-variation of amino-acid residues (top right), contact network inferred by network deconvolution (bottom left), contact network inferred by our method based on spectral templates (bottom right). (b) Fraction of the real contact edges between amino-acids recovered for each method as a function of the number of edges considered. (c) Counterpart of (b) for protein YES HUMAN.\red{The zero in 250 in the xlabel of plot (b) is missing.}}
		\vspace{-0.1in}
	\label{F:network_sparsification}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As figure of merit we use the F-measure \cite{manning2008introduction}, i.e. the harmonic mean of edge precision and recall, that solely takes into account the support of the recovered graph while ignoring the weights. In Fig.~\ref{F:comparison_traditional} we plot the performance of the three methods as a function of the number of filtered graph signals observed for filters $\bbH_1$ and $\bbH_2$, where each point is the mean F-measure over the 20 testing graphs. 

When considering a general graph filter $\bbH_1$ our method clearly outperforms the other two. For instance, when $10^5$ signals are observed, our average F-measure is $0.81$ while the measures for correlation and graphical lasso are $0.29$ and $0.25$, respectively. Moreover, of the three methods, our approach is the only consistent one, i.e., achieving perfect recovery with increasing number of observed signals. Although striking at a first glance, the deficient performance of graphical lasso was expected. For general filters $\bbH_1$, the precision matrix is given by $\bbC_x^{-1} = \bbH_1^{-2}$ which in general is neither sparse nor shares the support of $\bbS$, the GSO to be recovered. When analyzing the specific case of graph filters $\bbH_2$, where the precision matrix exactly coincides with the desired graph-shift operator, graphical lasso outperforms both our method and the correlation-based method. This is not surprising since graphical lasso was designed for the recovery of sparse precision matrices. Notice however that for large number of observations our method also achieves perfect recovery, i.e., F-measure equal to 1.
%In summary, whenever the observations perfectly match the assumptions of graphical lasso, this latter method is preferable even though our method still achieves perfect recovery for a larger number of observations. Nevertheless, in the more frequent case of general graph filters, our method clearly outperforms the two established benchmarks. 


\noindent\textbf{Comparison with GSP methods.} We compare the recovery using spectral templates with \cite{DongLaplacianLearning} and \cite{Kalofolias2016inference_smoothAISTATS16}, both methods designed to identify the (combinatorial) Laplacian of a graph when given a set of smooth graph signals. Small modifications can be made to our framework to accommodate for this setting, thus permitting a fair comparison. More precisely, in solving \eqref{E:SparseAdj_l1_obj_noisy_matrix_v2} we use the set of admissible shifts given by 
%
\begin{align}\label{E:def_S_combinatorial_laplacian}
\ccalS_{\rm L_c}  :=  \{ \bbS \, | \, S_{ij} \leq 0   \,\, \text{for} \,\,& i\!\neq\! j,  \;\;\bbS\! \in \! \ccalM_{+}^N, \;\; \bbS \bbone = \bbzero \}.
\end{align}
%
Moreover, in order to account for the smoothness of the observed signals in the unknown graph we sort the eigenvectors $\hbv_k$ of the sample covariance in increasing order of their corresponding eigenvalues, and we require the recovered eigenvalues $\bblambda$ to satisfy $\lambda_{i} \geq \lambda_{i+k} + \delta$ for all $i$, and fixed $k$ and $\delta$. In this way, we assign the frequencies with larger presence in the observed signals to low eigenvalues in the recovered Laplacian. Unless otherwise noted, we set $\delta = 0.1$ and $k = 3$.

We compare the three methods of interest on two different types of graphs and three different signal generation models. We consider the recovery of the Laplacian $\bbS = \bbL$ of Erd\H{o}s-R\'enyi (ER) graphs \cite{bollobas1998random} with $N \! = \! 20$ nodes and edge probability $p \! = \! 0.3$ as well as Barab\'asi-Albert preferential attachment graphs \cite{bollobas1998random} with $N \! = \! 20$ generated from $m_0 = 4$ initially placed nodes, where each new node is connected to $m=3$ existing ones. We consider three models for smooth graph signals: i) multivariate normal signals with covariance given by the pseudo-inverse of $\bbL$, i.e., $\bbx_1 \sim \ccalN(\bbzero, \bbL^{\dag})$; ii) white signals filtered through an autoregressive (diffusion) process, that is $\bbx_2 = (\bbI + \bbL)^{-1} \bbw$, where $\bbw$ is white; and iii) white signals passed through an exponential filter, $\bbx_3 = \exp(-\bbL) \bbw$. For each of the six settings considered (two graphs combined with three signal types) we generate 10 training graphs, 100 testing graphs, and for every graph we generate 1000 graph signals. The training set is used to set the parameters in \cite{DongLaplacianLearning} and \cite{Kalofolias2016inference_smoothAISTATS16}, and in our case it serves the purpose of selecting the best $\epsilon$ [cf.~\eqref{E:SparseAdj_l1_obj_noisy_matrix_v2}]. To increase the difficulty of the recovery task, every signal $\bbx$ is perturbed as $\hbx = \bbx + \sigma \, \bbx \circ \bbz$, for $\sigma = 0.1$ and where each entry of $\bbz$ is an independent standard normal random variable. We focus on three performance measures, namely, the F-measure as explained in the previous experiment, the $\ell_2$ relative error of recovery of the edges, and the $\ell_2$ relative error of recovery of the degrees. 
The performance achieved by each method in the testing sets is summarized in Table~\ref{Tab:comparison_methods}. In all but one case, our method attains the largest F-measures and the smallest errors for all the graphs and signal types considered. 

Finally, for the particular cases of Erd\H{o}s-R\'enyi graphs and signals $\bbx_1$ (inverse Laplacian), we replicate the above procedure varying the number of observed signals $P$ from $100$ to $1000$. For SpecTemp, we increase $k$ when the number of observations decreases to account for the noisier ordering of the eigenvectors in the sample covariance. In this experiment we use $k=5$ for $P \leq 400$, $k=4$ for $400<P<800$ and $k=3$ for $P \geq 800$. In Fig.~\ref{F:comparison_kalo_dong} we plot the associated $\ell_2$ edge recovery errors. Notice that for small number of observations, the method in \cite{Kalofolias2016inference_smoothAISTATS16} outperforms SpecTemp whereas the opposite is true when more signals are observed. This can be attributed to the fact that SpecTemp assumes no specific model on the smoothness of the signal, thus, when enough signals are observed our more agnostic, data-driven approach exhibits a clear performance advantage.

\subsection{Network sparsification}\label{Ss:Sim_network_sparsification}

%Thus far we have assumed that the spectral templates $\bbV$ are estimated from the sample covariance $\hbC_x$ of observed graph signals (cf. Section~\red{XX}). An alternative interpretation is that we obtain a particular graph-shift $\bbS' = \hbC_x$ from the graph signals and then look for another shift $\bbS$ with (approximately) the same eigenvectors that minimizes a cost function $f(\bbS)$. This second interpretation can be extended to general initial shifts $\bbS'$. Specifically, given a shift $\bbS'$ we can use our framework to obtain a different shift $\bbS$ with the same eigenvectors but with desirable properties. 


With reference to the network sparsification problem outlined in Section \ref{sssec_sparsify}, our goal here is to identify the structural properties of proteins from a mutual information graph of the co-variation between the constitutional amino-acids \cite{Marks2011proteins}; see \cite{FeiziNetworkDeconvolution} for details. For example, for a particular protein, we want to recover the structural graph in the top left of Fig.~\ref{F:network_sparsification}(a) when given the graph of mutual information in the top right corner. Notice that the structural contacts along the first four sub-diagonals of the graphs were intentionally removed to assess the capability of the methods in detecting the contacts between distant amino-acids. The graph recovered by network deconvolution \cite{FeiziNetworkDeconvolution} is illustrated in the bottom left corner of Fig.~\ref{F:network_sparsification}(a) whereas the one recovered using spectral templates (SpecTemp) is depicted in the bottom right corner of the figure. Comparing both recovered graphs, SpecTemp leads to a sparser graph that follows more closely the desired structure to be recovered. To quantify this latter assertion, in Fig.~\ref{F:network_sparsification}(b) we plot the fraction of the real contact edges recovered for each method as a function of the number of edges considered, as done in \cite{FeiziNetworkDeconvolution}. 
For example, if for a given method the 100 edges with largest weight in the recovered graph contain $40\%$ of the edges in the ground truth graph we say that the 100 top edge predictions achieve a fraction of recovered edges equal to $0.4$.
As claimed in \cite{FeiziNetworkDeconvolution}, network deconvolution improves the estimation when compared to raw mutual information data. Nevertheless, from Fig.~\ref{F:network_sparsification}(b) it follows that SpecTemp outperforms network deconvolution. Notice that when $\epsilon = 0$ [cf.~\eqref{E:SparseAdj_l1_obj_noisy_matrix_v2}] we are forcing the eigenvectors of $\bbS$ to coincide exactly with those of the matrix of mutual information $\bbS'$. However, since $\bbS'$ is already a valid adjacency matrix, we end up recovering $\bbS = \bbS'$. By contrast, for larger values of $\epsilon$ the additional flexibility in the choice of the eigenvectors allows us to recover shifts $\bbS$ that more closely resemble the ground truth. For example, when considering the top $200$ edges, the mutual information and the network deconvolution methods recover $36\%$ and $43\%$ of the desired edges, respectively, while our method for $\epsilon \! = \! 1$ achieves a recovery of $53\%$. In Fig.~\ref{F:network_sparsification}(c) we present this same analysis for a different protein and similar results can be appreciated.




==> sec_6_conclusions.tex <==
%!TEX root = Topology_inference.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SECTION: CONCLUDING REMARKS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}\label{S:Conclusions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With $\bbS=\bbV\bbLambda\bbV^T$ being the shift operator associated with the graph $\ccalG$, we studied the problem of identifying $\bbS$ (hence the topology of $\ccalG$) using a two-step approach under which we first obtain $\bbV$, and then use $\bbV$ as input to find $\bbLambda$. The problem of finding $\bbLambda$ given $\bbV$ was formulated as a sparse recovery optimization. Efficient algorithms based on convex relaxations were developed, and theoretical conditions under which exact and robust recovery is guaranteed were derived for the cases where $\bbS$ represents the adjacency or the normalized Laplacian of $\ccalG$. 
%
%\green{Leveraging recent results in GSP, a number of motivating setups where the eigenvectors $\bbV$ can be identified were discussed. Our main focus was on using as input a set of signal realizations that were assumed to be stationary in $\bbS$, which is a model that arises in, e.g., setups with linear network diffusion dynamics. It was shown that in this case $\bbV$ can be found as the eigenvectors of the sample covariance of the available set, so that several well-established methods for topology identification based on local and partial correlations can be viewed as particular instances of the proposed approach. To highlight the practical relevance of the proposed schemes we carried out numerical tests showing the effectiveness in recovering synthetic and real-world graphs.}
%
In identifying $\bbV$, our main focus was on using as input a set of graph signal realizations, which is a prominent setup in Network Science. Under the assumption that such signals resulted from \green{diffusion dynamics} on the graph or, equivalently, that they were stationary in $\bbS$, it was shown that $\bbV$ could be estimated from the eigenvectors of the sample covariance of the available set. As a consequence, several well-established methods for topology identification based on local and partial correlations can be viewed as particular instances of the approach here presented.
%
The practical relevance of the proposed schemes and the gains relative to existing alternatives were highlighted carrying out numerical tests with synthetic and real-world graphs.

%The motivating application was that of finding $\bbV$ as the eigenvectors of the sample covariance of a set of signal realizations. Under the assumption that those signals were stationary in $\bbS$, which is a model that arises in network diffusion dynamics, it was shown that the proposed method succesfully recover outperforming well-established methods based on local and partial correlations that can be viewed as particular instances of the proposed algorithm. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
%\noindent\red{Open issues (to-do, to-fix list):}
%
%\begin{itemize}
%	\red{\item Revisar el apartado de notacion al final de la Section \ref{S:Introduction}.
%	\item Figure in Section \ref{S:prelim_problem} is missing. I think that we can generate one direct vs indirect relationships, is not what Alejandro wanted but it can be useful.
%\item While \eqref{eqn_shift_operator_normal} uses conjugate-transpose (Hermitian), the formulations in e.g., \eqref{eqn_zero_norm} uses
%	transpose. I think that everything holds if we replace $^T$ with $^H$ right? The lambdas will be complex, but writing each of them as a tuple (real and imaginary), the optimization is still convex. I do not know about the theorems. } 
%	\end{itemize}
%	

